Line Failure Localization of Power Networks Part I: Non-cut Outages

Transmission line failures in power systems propagate non-locally, making the control of the resulting outages extremely difficult. In this work, we establish a mathematical theory that characterizes the patterns of line failure propagation and localization in terms of network graph structure. It provides a novel perspective on distribution factors that precisely captures Kirchhoff's Law in terms of topological structures. Our results show that the distribution of specific collections of subtrees of the transmission network plays a critical role on the patterns of power redistribution, and motivates the block decomposition of the transmission network as a structure to understand long-distance propagation of disturbances. In Part I of this paper, we present the case when the post-contingency network remains connected after an initial set of lines are disconnected simultaneously. In Part II, we present the case when an outage separates the network into multiple islands.

==> App-representation.tex <==
%\cliang{Revisit.}
In this section we collect several spectral properties that follow from Theorem \ref{prop:prem_basis}.
\subsection{Inverse of Reduced Laplacian Matrix}
\begin{cor}
For all $i,j\in\calN$ we have $
A_{ij} \ge 0$, and equality holds if and only if every path from $i$ to $j$ contains the reference node $n$.
\end{cor}
\begin{proof}
The statement trivially holds when $i$ or $j$ coincides with $n$, so in the rest of the proof we focus on the case $i,j \neq n$. In this case, since $\chi(E) \ge 0$ for all $E$, we clearly have $A_{ij} \ge 0$ and equality holds if and only if the set $\calT(ij,n)$ is empty.

If every path from $i$ to $j$ contains $n$, then since any tree containing $\set{i,j}$ induces a path from $i$ to $j$, we know that this tree also contains $n$. As a result, $\calT(ij, n) = \emptyset$. Conversely, if $\calT(ij, n) = \emptyset$, then any path from $i$ to $j$ must contain $n$, since for any path from $i$ to $j$ not passing through $n$, we can iteratively add edges that do not have $n$ as an endpoint to obtain a spanning tree over the nodes set $\calN\bs \set{n}$. This tree together with the node $n$ itself is an element of $\calT(ij, n)$. We thus have shown that $\calT(ij, n)$ is empty if and only if every path from $i$ to $j$ contains $n$. %This completes the proof.
\end{proof}


\subsection{Effective Reactance}

The Laplacian matrix $L$ appears in circuit analysis as the admittance matrix (with a different weight), which explicitly relates the voltage and current vectors in an electrical resistive network \cite{dorfler2013kron}. In particular, given a network of resistors, it is shown in \cite{dorfler2013kron} that the \textit{effective resistance} between two nodes $i$ and $j$ can be computed as
\begin{equation}\label{eqn:prem_effective_reactance}
R_{ij}:=L^\dagger_{ii}+L^\dagger_{jj}-L^\dagger_{ij}-L^\dagger_{ji},
\end{equation}
where $L^\dagger$ is the Penrose-Moore pseudoinverse of $L$. With an analogous calculation, we can show that in our setting \eqref{eqn:prem_effective_reactance} gives the \textit{effective reactance} between the buses $i$ and $j$. This means that, assuming we connect the buses $i$ and $j$ (with phase angles $\theta_i$ and $\theta_j$ respectively) to an external probing circuit, when there are no other injections in the network, the branch flow $f_{ij}$ (from the external circuit) into bus $i$ and out of bus $j$ (into the external circuit) is given as
$$
f_{ij}=\frac{\theta_i-\theta_j}{R_{ij}}.
$$
Therefore, the network can be equivalently reduced to a single line with reactance $R_{ij}$. If $(i,j)\in\calE$, the reactance of $(i,j)$ is given as $X_{ij}:= 1/B_{ij}$. Physical intuition then suggests that $R_{ij} \le X_{ij}$, as additional paths from $i$ to $j$ in the network should only decrease the overall reactance. We now give a graphical interpretation for the difference $X_{ij}-R_{ij}$ and use it to prove this result rigorously.
\begin{cor}\label{cor:prem_effective_reactance}
For all $(i,j)\in\calE$ we have
  $$
 X_{ij}-R_{ij}=X_{ij}\cdot\frac{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\beta(E)}{\sum_{E\in \calT_\calE}\beta(E)}.
  $$
  In particular, $X_{ij}\ge R_{ij}$ and the inequality is strict if and only if the graph $\calG$ is still connected after removing $(i,j)$.
\end{cor}
\begin{proof} 
The proof uses the following relation between $L^\dagger$ and $A$.%\slow{Is the following relation known in the literature and we can just cite without proof?} \cliang{I did not find a suitable reference...} 
%\ale{Isn't Lemma 16 essentially Lemma 2?} \cliang{Lemma 16 is a special case of Lemma 2. We do not require either $(i,j)$ or $(\hat i, \hat j)$ is an edge.}
\begin{lemma}\label{lemma:prem_l_a_equiv}
For every edge $(i,j)\in\calE$ we have
$$
L^\dagger_{ii}+L^\dagger_{jj}-L^\dagger_{ij}-L^\dagger_{ji}=A_{ii}+A_{jj}-A_{ij}-A_{ji}.
$$
\end{lemma}
\begin{proof}[Proof of the lemma]
We know that if the equation $p=L\theta$ is solvable, the solution $\theta$ is unique after quotienting away the kernel of $L$, which is given by $\spann\paren{\bff{1}}$. Noting that the latter coincides with the kernel of $C^T$, we conclude that the vector $f=BC^T\theta$ is uniquely determined.

To prove the desired identity, we will equate two alternative formulas for the branch flows $f$. The first one relies on the fact that $L^\dagger p$ always gives a feasible $\theta$ and, therefore,
\begin{equation}\label{eqn:prem_pseudoinverse}
f=BC^TL^\dagger p.
\end{equation}
The second way to calculate $f$ is to set the phase angle at the reference node to zero, which indirectly implies that
$$
\tilde{\theta} = \begin{bmatrix} \ol{\theta} \\ 0 \end{bmatrix}= \begin{bmatrix} \ol{L}^{-1}\ol{p}  \\ 0 \end{bmatrix}= Ap,
$$
where $\ol{\theta}$ and $\ol{p}$ are the vector of non-reference node phase angles and injections. We then have
\begin{equation}\label{eqn:prem_submatrix}
f=BC^T\tilde{\theta}= BC^TA p.
\end{equation}
Now take $i, j \in\calN$. Setting the injections $p_i=-p_j=1$ and zero elsewhere, by equating the branch flow $f_{ij}$ computed from \eqref{eqn:prem_pseudoinverse} and \eqref{eqn:prem_submatrix}, we obtain that
$$
L^\dagger_{ii}+L^\dagger_{jj}-L^\dagger_{ij}-L^\dagger_{ji}=A_{ii}+A_{jj}-A_{ij}-A_{ji}. \qedhere
$$
\end{proof}
In other words, we can replace the $L^{\dagger}$'s in equation~\eqref{eqn:prem_effective_reactance} by the matrix $A$, which allows us to apply Theorem \ref{prop:prem_basis}.

Now by taking $\hat{i}=i$, $\hat{j}=j$ in Theorem \ref{cor:prem_cross_product} and applying Lemma \ref{lemma:prem_l_a_equiv}, we see that
$$
R_{ij}=A_{ii}+A_{jj}-2A_{ij}=\frac{\sum_{E\in\calT(i,j)}\beta(E)}{\sum_{E\in \calT_\calE}\beta(E)}.
$$
For each forest in $\calT(i,j)$, we can add the edge $(i,j)$ to form a spanning tree passing through $(i,j)$. Conversely, each spanning tree passing through $(i,j)$ after removing the edge $(i,j)$ produces a forest in $\calT(i,j)$. By definition of $\beta(E)$, this fact implies that
$$
\sum_{E\in\calT(\set{i},\set{j})}\beta(E)=X_{ij}\sum_{E\in\calT'}\beta(E),
$$
where $\calT'$ denotes the set of all spanning trees passing through $(i,j)$. Therefore,
\begin{IEEEeqnarray*}{rCl}
X_{ij}-R_{ij}&=&X_{ij}\cdot\frac{\sum_{E\in \calT_\calE}\beta(E)-\sum_{E\in\calT'}\beta(E)}{\sum_{E\in \calT_\calE}\beta(E)}\\
&=&X_{ij}\cdot\frac{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\beta(E)}{\sum_{E\in \calT_\calE}\beta(E)},
\end{IEEEeqnarray*}
and the proof is completed.
\end{proof}


From Corollary \ref{cor:prem_effective_reactance}, we see that for an edge $(i,j)$, the reduction ratio of its reactance coming from the network is precisely the portion of weighted spanning trees not passing through $(i,j)$ among all spanning trees. 
%In other words, $R_{ij}=\frac{\sum_{E\in\calT_{ \set{(i,j)}}}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)} X_{ij}$, i.e. $R_{ij}$ is proportional to the fraction of weighted spanning trees passing through edge $(i,j)$.
Thus, more connections from the network leads to more reduction in the effective reactance on $(i,j)$, which agrees with our physical intuition.

We remark that this reactance reduction ratio is closely related to the \textit{spanning tree centrality measure} \cite{teixeira2013spanning}. Indeed,
$$
\frac{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)} + c_{(i,j)} = 1,
$$
where $c_{(i,j)}$ is the spanning tree centrality of $(i,j)$. As a result
$$
R_{ij} = X_{ij}c_{(i,j)},
$$
which means that in a power network the spanning tree centrality $c_{(i,j)}$ of a transmission line $(i,j)$ precisely captures the ratio between its effective reactance $R_{ij}$ and its physical line reactance $X_{ij}$.



==> SpectralRep.tex <==
%

==> basic.tex <==
%The tree-partition of a power system graph has emerged as a powerful tool in cascading failure analysis. 
%In this section, we define the tree partition motivated by the Simple Loop Criterion from the last section, discuss its uniqueness and show that the ``finest'' tree partition of a general graph can be computed in linear time.
\begin{figure}
\centering
\iftoggle{isarxiv}{
\includegraphics[width=0.35\textwidth]{arxiv_figs/tree_partition.eps}
}{
\includegraphics[width=0.35\textwidth]{figs/tree_partition.png}
}
\caption{The construction of $\calG_\calP$ from $\calP$.}\label{fig:tree_partition}
\end{figure}

%To start with, we first formally define the concept of tree-partition. 
For a power network $\calG=(\calN,\calE)$, a collection $\calP=\set{\calN_1,\calN_2,\cdots, \calN_k}$ of subsets of $\calN$ is said to form a \emph{partition} of $\calG$ if $\bigcup_{i=1}^k \calN_i=\calN$ and $\calN_i\cap\calN_j=\emptyset$ for $i\neq j$.

Given a partition $\calP=\set{\calN_1,\calN_2,\cdots, \calN_k}$ of $\calG$ 
we define a \textit{reduced multi-graph} $\calG_\calP$ as follows (see Fig.~\ref{fig:tree_partition}).
First, $\calG_\calP$ has $k$ nodes, one for each subset $\calN_i$; we often use $\calN_i$ to identify the nodes of  $\calG_\calP$.
% we reduce each subset $\calN_i$ (and all its internal edges) to a ``super node'' . The collection of all super nodes forms the node set of $\calG_\calP$. 
Second, there is an undirected edge connecting the nodes $\calN_i$ and $\calN_j$ of $\calG_\calP$ for every pair
of nodes $v \in\calN_i$, $w\in\calN_j$ in the original graph $\calG$ that are adjacent in $\calG$, i.e., 
$(v, w)\in\calE$.
There are multiple edges between nodes $\calN_i$ and $\calN_j$ of $\calG_\calP$ 
when multiple pairs of such nodes $(v, w)$ exist in the original graph $\calG$. 
Unlike the graph $\calG$ (to which we have assigned an arbitrary orientation), the reduced multi-graph $\calG_\calP$ is undirected.

\begin{defn}
A partition $\calP=\set{\calN_1,\calN_2,\cdots,\calN_k}$ of $\calG$ is a \textbf{tree partition} if the reduced graph $\calG_\calP$ is a tree. The sets $\calN_i$ are referred to as \textbf{regions} of $\calP$. An edge $e \in \calE$ with both endpoints inside the same region $\calN_i$ is said to be \textbf{within} $\calN_i$ and it is called a \textbf{bridge}\footnote{We remark that our definition of bridges agrees with the classical definition of bridges in graph theory (i.e., the removal of any such edge disconnects the original graph) in the sense that if the tree partition $\calP$ is irreducible (see Definition \ref{defn:irreducible} later) any bridge defined in our sense is a bridge in the classical sense, and vice versa.} otherwise. We denote by $\calE_i$ the set of edges within $\calN_i$ and by $\calE_b$ the set of bridges, so that 
$
	\calE = \calE_b \cup \bigcup_{i=1}^k \calE_i.
$
\end{defn}

A tree partition is exhibited in Fig.~\ref{fig:tree_partition} for the specific graph. Other tree partitions of the same graph exist: for instance, one can always consider the trivial partition $\calP_0=\set{\calN}$, in which all the nodes are collapsed into a single region. The tree partition of a network $\calG$ is thus not unique in general.  Nevertheless, if we require the tree partition to be as ``fine'' as possible, such a partition is unique.

Specifically, given a graph $\calG$, we define a partial order $\succeq$ over the set of all tree partitions of $\calG$ (which is nonempty as it always contains the trivial partition $\calP_0$) as follows. For two tree partitions $\calP^1=\set{\calN_1^1,\calN_2^1,\cdots,\calN_{k_1}^1}$ and $\calP^2=\set{\calN_1^2,\calN_2^2,\cdots,\calN_{k_2}^2}$, we say $\calP^1$ is \emph{finer} than $\calP^2$, denoted as $\calP^1\succeq \calP^2$, if for any $i=1,2,\ldots, k_1$, there exists some $j(i)\in \set{1,2,\ldots, k_2}$ such that $\calN_i^1\subseteq \calN_{j(i)}^2$. That is, $\calP^1$ is finer than $\calP^2$ if each region in $\calP^1$ is contained in some region in $\calP^2$ (see Fig.~\ref{fig:partition_order}). It is easy to check that $\succeq$ is in fact a partial order over all possible tree partitions of $\calG$.
%\slow{In Fig 6 caption, should the region $\calN^2_2$ be $\calN^1_2$?  Also, in Definition 12, if there are two edges between two nodes in $\calG_p$, is that still a tree partition?  If not, then is $\calP_1$ in FIg 6 a tree partition even though there are two edges between the two regions? Or is it a partition, but not tree partition?}
%\cliang{There was a mistake in Fig. 6.  I have fixed the figure.}

\begin{defn}\label{defn:irreducible}
A tree partition $\calP$ is said to be \textbf{irreducible} if $\calP$ is maximal with respect to the partial order $\succeq$.
\end{defn}

In other words, an irreducible tree partition is a tree partition of $\calG$ that cannot be made finer.

\begin{prop}\label{prop:unique_irreducible}
For any graph $\calG$, the irreducible tree partition of $\calG$ is unique.
\end{prop}
\iftoggle{isreport}{See Appendix \ref{proof:uniqueness} for a proof.}{See our online report \cite{part1} for a proof.}
\begin{figure}[t]
\centering
\iftoggle{isarxiv}{
\includegraphics[width=.275\textwidth]{arxiv_figs/partition_order.eps}
}{
\includegraphics[width=.275\textwidth]{figs/partition_order.png}
}
\caption{An illustration of the partial order $\succeq$ over tree partitions. The partition $\calP^1=\set{\calN_1^1, \calN_2^1, \calN_3^1, \calN_4^1}$ is finer than $\calP^2=\set{\calN_1^2, \calN_2^2}$.}\label{fig:partition_order}
\end{figure}
We remark that our proof of Proposition \ref{prop:unique_irreducible} not only shows that the irreducible tree partition of $\calG$ is unique, but also implies that the problem of computing this unique irreducible tree partition reduces to finding all the bridges of $\calG$. We can thus adapt Tarjan's bridge-finding algorithm \cite{tarjan1974note} and devise an algorithm that computes the irreducible tree partition of $\calG$ in $O(n+m)$ time, as we summarize in Algorithm \ref{alg:tree_partition} below (see also the proof of Proposition \ref{prop:unique_irreducible} in\iftoggle{isreport}{ Appendix \ref{proof:uniqueness}}{~\cite{part1}} for more details).

\begin{algorithm}
\caption{Irreducible Tree Partition Finding Algorithm}\label{alg:tree_partition}
\begin{algorithmic}[1]
    \STATE Execute Tarjan's bridge-finding algorithm \cite{tarjan1974note} on $\calG=(\calN,\calE)$ to compute the set of bridges $\calE_b$.
    \STATE Remove edges in $\calE_b$ from $\calE$ to form the partitioned graph $(\calN, \calE\bs\calE_b)$.
    \STATE Breadth-first search on the partitioned graph $(\calN,\calE\bs\calE_b)$ to compute its set of connected components $\calP:=\set{C_1, C_2, \ldots, C_k}$. Return $\calP$.
     \end{algorithmic}
\end{algorithm}

==> bridge.tex <==
The remaining case necessary to prove Theorem \ref{thm:summary} is a characterization of the power flow redistribution when a bridge is tripped.  Here, we show that such failures generally propagate through the entire network.

Recall that, when $e$ is not a bridge, the branch flow change on $\hat{e}$ due to tripping $e$ is given by
\begin{equation}\label{eqn:power_change}
\Delta P_{\hat{e}} = K_{e\hat{e}} \times P_e.
\end{equation}
When $e$ is a bridge, tripping $e$ disconnects the power grid into two components, and the power in each connected component may not be balanced. Such power imbalance can be resolved by a power balance rule $\calB$ (see \cite{bernstein2014power,bienstock2010n-k,bienstock2011control,bernstein2014vulnerability} for examples of such rules), which together with the DC model uniquely determines the new branch flows (and thus the branch flow change $\Delta P_{\hat{e}}$). We extend the definition of $K_{e\hat{e}}$ through \eqref{eqn:power_change} to the case where $e$ is a bridge and call it the \emph{extended line outage distribution factor}. Besides being related to the $B$ and $C$ matrices, this extended $K_{e\hat{e}}$ factor also depends on the power injection $p$ and the power balance rule $\calB$.

Power networks without microgrids typically operate in ``island-free mode'' as islanding (i.e.,~isolating a part of the grid power flow from the rest of the network) poses a safety hazard to utility maintainence and repair personnel and potentially leads to damage of the infrastructure \cite{ropp1999analysis}. Formally we define the concept of island-free as follows. 

\begin{defn}\label{defn:island_free}
For a power network $\calG$, an injection $p$ is said to be \textbf{island-free} if under the injection $p$, the branch flow $P$ in $\calG$ satisfies $P_e\neq0$ for any bridge $e$.
\end{defn}

Intuitively, island-free means that no part of the grid balances its own power.

 For a grid $\calG$ operating with the balance rule $\calB$, when a net power imbalance of level $M$ is detected, the rule $\calB$ selects a set of \emph{participating} buses from $\calG$ and adjust their injections properly to cancel $M$. The rules studied in the literature \cite{soltan2015analysis,bernstein2014power,bienstock2010n-k,bienstock2011control,bernstein2014vulnerability} are typically \emph{linear} in the sense that, for any participating bus $j$, the injection adjustment $\delta p_j$ dictated by the rule $\calB$ is linear in $M$.

Denote the set of participating buses of $\calB$ as $\calN_{\calB}$ and let $n_b=\abs{\calN_{\calB}}$. The rule $\calB$ can then be interpreted as a linear transformation from $\R$ to $\R^{n_b}$ given by
$$
\calB(M) = \paren{\alpha_j M: j\in\calN_{\calB}},
$$
where $\alpha_j$ are positive constants that sum to $1$. For instance, if the imbalance is uniformly absorbed by the generators as in \cite{bernstein2014power,soltan2015analysis}, we have $\calN_{\calB}$ to be the set of generators and $\alpha_j=1/G$, where $G$ is the number of generators. As another example, if the imbalance is regulated through Automatic Generation Control, then we have $\calN_{\calB}$ to be set of controllable generators and $\alpha_j$ are the normalized generator participation factors.

\begin{defn}\label{defn:participating}
For a power grid $\calG$ with tree partition $\calP=\set{\calN_1,\calN_2,\cdots, \calN_k}$ operating under power balance rule $\calB$, a region $\calN_i$ with block decomposition $\set{\calC_{1}^i, \calC_2^i, \cdots, \calC_{m_i}^i}$ is said to be a \textbf{participating region} if $\calN_{\calB}\cap \calC^i_j$ contains a non-cut-vertex for $j=1,2,\ldots, m_i$. The grid $\calG$ is said to be a \textbf{participating grid} if $\calN_i$ is participating for  $i=1,2,\ldots,k$.
\end{defn}

A power grid is usually participating. For instance, if $\calB$ allocates the power imbalance uniformly to the generators as in \cite{bernstein2014power,soltan2015analysis}, as long as each cell in the network contains a generator that is not at the ``gate'' (i.e., it is not a cut vertex\footnote{A cut vertex is always at the ``gate'' of a cell as all paths from outside towards vertices in the cell must pass through a cut vertex\cite{harary1969graph}.}), the grid is participating. If in addition load-side participation is exploited and $\calB$ also allocates the power imbalance to controllable loads, then the power grid is participating if the controllable loads are ubiquitously deployed to all buses. 

Given the above, we now state our main result.

\begin{prop}\label{prop:bridge_prop}
Consider a participating power network $\calG$ with island-free injection $p$ and under line susceptance perturbation $\mu$ that is absolutely continuous with respect to $\calL_m$. If $e$ is a bridge of $\calG$, then for any $\hat{e}\neq e$, we have
$$
\mu(K_{e\hat{e}}\neq 0)=1.
$$
\end{prop}
\iftoggle{isreport}{
See Appendix \ref{proof:bridge_prop} for a proof.
}{
See our online report for a proof \cite{report}.
}

The proof of Proposition \ref{prop:bridge_prop} provides interesting insights. In particular, both the participating grid and island-free injection conditions are in fact necessary. For instance, if the supply and demand is balanced within a region (which violates the island-free condition), then when the bridge connecting this region to other parts of the grid is tripped, the power is still balanced and thus the power flow within the region stays unchanged. This is precisely the case when a microgrid is connected to the power network: by disconnecting the microgrid from the main grid (which effectively trips a bridge in the original system), branch flows within both the microgrid and the main grid are not impacted.

Note that the result in Proposition \ref{prop:bridge_prop} can be easily extended to more general settings. It is straightforward to extend our proof to cover the case where neither condition is posed. We prefer not to present this generalization here because it would unnecessarily complicate the proof of the result without providing new insights.% and because, as mentioned earlier, in a typical grid operation scenario both conditions are satisfied. 

==> bridge_prop_proof.tex <==
\begin{figure}
\centering
\iftoggle{isarxiv}{
\includegraphics[width=.35\textwidth]{localized_graph.png}
}{
\includegraphics[width=.35\textwidth]{figs/localized_graph.png}
}
\caption{The localized graph $\calG_{\calN_1}$. $\calN_t$ is the imaginary bus containing $e$ and $\calN_{1,i}$'s are remaining imaginary buses. The power adjustments from the power balance rule $\calB$ are shown near each participating bus in reaction to a power loss of $M$.}\label{fig:localized}
\end{figure}
Denote the two connected components of $\calG$ after $e$ is tripped as $D_1,D_2$. Since the injection is island-free, we know $\sum_{j\in D_1}p_i\neq 0$ and $\sum_{j\in D_2}p_i\neq 0$, and thus the power is not balanced in neither $D_1$ nor $D_2$. We will show that $K_{e\hat{e}}\neq 0$ for any $\hat{e}$ within $D_1$. The case where $\hat{e}$ belongs to $D_2$ can be addressed similarly.

First we consider the case where $\hat{e}$ is a bridge. Denote the two connected components of $D_1$ after removing $\hat{e}$ as $D_{1,1}$ and $D_{1,2}$, and without loss of generality assume $D_{1,2}$ is originally connected to $e$ in $\calG$. It is easy to see that the branch flow change on $\hat{e}$ is given by
$$
\Delta P_{\hat{e}} = \sum_{j\in D_{1,1}}\delta p_j \neq 0
$$
where the last $\neq$ is because the grid is participating and thus all tree partition regions in $D_{1,1}$ would adjust their injections (in the same ``direction'' as $\alpha_j$'s are positive). As a result we see $K_{e\hat{e}}=\Delta P_{\hat{e}}/P_e\neq 0$.

Next we consider the case where $\hat{e}$ is not a bridge. In this case, $\hat{e}$ belongs to a certain tree partition region, say $\calN_1$. Let $n_1,n_2,\cdots, n_l$ be the set of participating buses in $\calN_1$. By collapsing all regions other than $\calN_1$, we can define a localized graph $\calG_{\calN_1}$ centered around $\calN_1$ as shown in Fig.~\ref{fig:localized}. Specifically, for each bridge $b$ incident to $\calN_1$, we create an imaginary bus that aggregates all injections inside all tree partition regions that can be reached by $\calN_1$ through $b$ \emph{before} $e$ is tripped, and this imaginary bus is connected to $\calN_1$ via the corresponding bridge $b$. If $e$ is not directly incident to $\calN_1$, then $e$ must connect two regions that are collapsed to a common imaginary bus, say $\calN_t$. If $e$ is incident to $\calN_1$ and its end point in $\calN_1$ is $n_e$, then we let $\calN_t$ be an additional imaginary bus that is connected to $n_e$ to mimic the edge $e$ (that is, before $e$ is tripped, this imaginary bus $\calN_t$ supplies power $P_e$ towards $n_e$ and after $e$ is tripped, $\calN_t$ loses all its injection; moreover the edge connecting $\calN_t$ to $n_e$ has susceptance $B_e$). Denote other imaginary buses as $\calN_{1,1},\calN_{1,2},\cdots, \calN_{1,q}$. 

Without loss of generality, let us assume because of the tripping of $e$, the aggregate power in $D_1$ is in shortage of $M$. Then the enforcement of the power balance rule $\calB$ would increase the power injection at each participating bus in $D_1$, which translates to the power adjustment as demonstrated in Fig.~\ref{fig:localized}. Specifically, the injection at $\calN_t$ would drop by $\alpha_{\calN_t}M$ as the power flow from $e$ is lost (the drop is generally not $M$ unless $e$ is directly incident to $\calN_1$); the injections at $\calN_{1,1},\calN_{1,2}, \cdots, \calN_{1,q}$ increase by $\alpha_{\calN_{1,i}} M$; and injections at the participating buses $n_1,n_2,\cdots, n_l$ in $\calN_1$ increase by $\alpha_{n_i}M$. In other words, by rebalancing power according to the rule $\calB$, we effectively shift the injections from $\calN_t$ to $\calN_{1,1},\calN_{1,2}, \cdots, \calN_{1,q}$ and $n_1,n_2,\cdots, n_l$.

Let the set of edges in $\calG_{\calN_1}$ be $\calE_1$. Pick $\calN_t$ to be the slack bus in this localized graph $\calG_{\calN_1}$ and define an index set
$$
\calI:=\set{\calN_{1,1},\calN_{1,2}, \cdots, \calN_{1,q}, n_1,n_2,\cdots, n_l}
$$
For any $i\in\calI$, let $g^{i}(B)$ be the following polynomial in line susceptances $(B_e:e\in\calE_1)$ 
$$
\sum_{E\in\calT_{\calE_1}\paren{\set{i,w},\set{\calN_t,z}}}\chi(E) - \sum_{E\in\calT_{\calE_1}\paren{\set{i,z},\set{\calN_t,w}}}\chi(E)
$$
where $\calT_{\calE_1}\paren{\calN_1,\calN_2}$ is the set of spanning forests of $\calG_{\calN_1}$ consisting of exactly two trees that contain $\calN_1$ and $\calN_2$ respectively (see Section \ref{section:model} for more details on the corresponding notion in $\calG$). By Proposition V.3 from our previous work \cite{guo2017monotonicity}, the branch flow change on $\hat{e}$ coming from the power shift from $\calN_t$ with amount $\alpha_iM$ towards $i$ is given by
$$
\Delta P^{i}_{\hat{e}}=\alpha_{i}M \times \frac{g^{i}(E)}{\sum_{E\in\calT_{\calE_1}}\chi(E)}
$$
where $\calT_{\calE_1}$ denotes the set of all spanning trees of $\calG_{\calN_1}$. Put
$$
g(B):=\sum_{i\in\calI}\alpha_{i}g^{i}(B)
$$
By linearity, we know
$$
\Delta P_{\hat{e}}=M\times \frac{g(B)}{\sum_{E\in\calT_\calE}\chi(E)}
$$

We claim $g(B)$ is not identically zero. Indeed, by a similar argument to the proof of Proposition \ref{prop:same_region}, we know that for any $i,j\in\calI$ (including the case $i=j$), the following is true:
$$
\calT_{\calE_1}\paren{\set{i,w},\set{\calN_t,z}}\cap \calT_{\calE_1}\paren{\set{j,z},\set{\calN_t,w}}=\emptyset
$$
As a result, a term in $g^i(B)$ with coefficient $1$ is never canceled by a term in $g^j(B)$ with coefficient $-1$, and vice versa. Therefore, to show $g(B)$ is not identically zero, it suffices to show at least one of $g^i(B)$ is not identically zero.

To do so, let $\calC$ be the cell that contains $\hat{e}$. Since $\calN_1$ is participating with respect to $\calB$, we know there exists a bus within $\calC$, say $n_1$, that participates the power balance and is not a cut vertex. Recall that any path from $\calN_t$ to $\calC$ must go through a common cut vertex in $\calC$ \cite{harary1969graph}, say $n_e$. Now by adding an edge between $n_e$ and $n_1$ (if it does not exist originally), the resulting cell $\calC'$ is still 2-connected. Thus there exists a simple loop in $\calC'$ that contains the edge $(n_e,n_1)$ and $\hat{e}=(w,z)$, which implies we can find two disjoint paths $P_1$ and $P_2$ connecting the endpoints of these two edges. Without loss of generality, assume $P_1$ connects $n_e$ to $w$ and $P_2$ connects $n_1$ to $z$. By concatenating the path from $\calN_t$ to $n_e$, we can extend $P_1$ to a path $\tilde{P}_1$ from $\calN_t$ to $w$, which is still disjoint from $P_2$. Now, by iteratively adding edges, we can extend $\tilde{P}_1$ and $P_2$ to a spanning forest of $\calG_{\calN_1}$ consisting of exactly two trees, which is an element of $\calT_{\calE_1}\paren{\set{n_1,z},\set{\calN_t,w}}$. This in particular implies $g^{n_1}(B)$ is not identically zero and therefore $g(B)$ is not identically zero.

Again by the classical algebraic geometry result asserting the root set of any polynomial that is not identically zero has Lebesgue measure zero\cite{federer1969geometric}, and because of the absolute continuity of $\mu$, we know
$$
\mu\paren{\Delta P_{\hat{e}}=0}=\calL_m\paren{g(B+\omega)=0}=0
$$
and thus
$$
\mu\paren{K_{e\hat{e}}\neq 0}=\mu\paren{\Delta P_{\hat{e}}\neq 0} = 1
$$
This completes our proof. \qedd

==> case_study.tex <==
Our findings highlight a new approach for improving the robustness of the network. More specifically, Theorem~\ref{thm:summary} and the discussion in Section~\ref{section:non-bridge} suggest that it is possible to localize failure propagation by \emph{temporarily} switching off certain transmission lines based on the specific injection. This creates more, smaller areas where failure cascades can be contained.  We remark that the lines that are switched off are still part of the system. In cases where the newly created bridges are tripped, some of these lines should be switched on so the system are still connected.  The examples presented below are preliminary and we are still investigating how to optimally tradeoff the increased robustness from localized failures and the yet also increased vulnerability from having more bridges.
 
It is reasonable to expect that such an action may increase the stress on the remaining lines and, in this way, worsen the network congestion. In fact, one may expect that improved system robustness obtained by switching off lines \textit{always} comes at the price of increased congestion levels. In this section, we argue that this is not necessarily the case, and show that if the lines to switch off are selected properly, it is possible to \emph{improve the system robustness and reduce the congestion simultaneously.} We corroborate this claim by considering first a small stylized example and then an IEEE test system.

\subsection{Double-Ring Network}
\begin{figure}
\centering
\iftoggle{isarxiv}{
\subfloat[]{\includegraphics[width=.22\textwidth]{double_ring.png}
}
\hspace{0.2cm}
\subfloat[]{\includegraphics[width=.22\textwidth]{double_ring_trip.png}
}
}{
\subfloat[]{\includegraphics[width=.22\textwidth]{figs/double_ring.png}
}
\hspace{0.2cm}
\subfloat[]{\includegraphics[width=.22\textwidth]{figs/double_ring_trip.png}
}
}
\caption{(a) A double-ring network. $G$ is the generator bus and $L$ is the load bus. Arrows represent the original power flow. (b) The new network after removing an edge. Arrows represent the new power flow.}\label{fig:double_ring}
\end{figure}

%We start by looking at an example where it is possible to improve the system robustness to cascades and congestion management \emph{simultaneously}. 
Consider the double-ring network in Fig.~\ref{fig:double_ring}(a), which contains exactly one generator and one load bus. The original power flow on this network is also shown in Fig.~\ref{fig:double_ring}(a). Suppose we switch off the upper tie-line. The new network and the redistributed power flow are shown in Fig.~\ref{fig:double_ring}(b). In this example, by switching off one transmission line, the circulating flows inside the hexgons are removed and the overall network congestion is decreased. In fact, it is easy to show that the topology in Fig.~\ref{fig:double_ring}(b) minimizes the sum of (absolute) branch flows over all possible topologies.%\footnote{This is a result of the Max-Flow-Min-Cut theorem. Indeed, for any ``flow'' from $G$ to $L$ of ``volume'' $d$, where $d$ is the demand of $L$, there exists a ``cut edge set'' such that the sum of ``flows'' on this set is exactly $d$. See  \cite{dantzig2003max} for the definition of these terminologies and a proof to the theorem.}.

\subsection{IEEE test system}

\begin{figure*}[t]
\centering
\iftoggle{isarxiv}{
\subfloat[Original influence graph.]{
\includegraphics[width=.83\textwidth]{inf_graph_before.png}
}
\hfill
\subfloat[The influence graph after switching off $e_1$, $e_2$ and $e_3$. The black dashed line indicates the failure propagation boundary defined by the tree partition. The vertices $c_1$ and $c_2$ are cut vertices.]{
\includegraphics[width=.83\textwidth]{inf_graph_after.png}
}
}{
\subfloat[Original influence graph.]{
\includegraphics[width=.83\textwidth]{figs/inf_graph_before.png}
}
\hfill
\subfloat[The influence graph after switching off $e_1$, $e_2$ and $e_3$. The black dashed line indicates the failure propagation boundary defined by the tree partition. The vertices $c_1$ and $c_2$ are cut vertices.]{
\includegraphics[width=.83\textwidth]{figs/inf_graph_after.png}
}
}
\caption{Influence graphs on the IEEE 118-bus network before and after switching off lines $e_1$, $e_2$ and $e_3$. Blue edges represent physical transmission lines and grey edges represent connections in the influence graph.}\label{fig:inf_graph}
\end{figure*}

In the simple example above, removing a line provides improvements in both robustness and congestion. Now, we move to the case of a more realistic network, the IEEE 118-bus test system. In this case, we also see that line removals can improve robustness without more than minor increase in congestion.

In our experiments, the system parameters are taken from the Matpower Simulation Package \cite{zimmerman2011matpower} and we plot the influence graphs among the transmission lines to demonstrate how a line failure propagates in this network\footnote{The original IEEE 118-bus network has some trivial ``dangling'' bridges that we remove (collapsing their injections to the nearest bus) to obtain a more transparent influence graph.}. More specifically, in the influence graph we plot, two edges $e$ and $\hat{e}$ are connected if the impact of tripping $e$ on $\hat{e}$ is not negligible (we use $|K_{e\hat{e}}|\geq 0.005$ as a threshold). In Fig.~\ref{fig:inf_graph}(a), we plot the influence graph of the original network. It can be seen that this influence graph is very dense and connects many edges that are topologically far away, showing the non-local propagation of line failures within this network.

Next, we switch off three edges (indicated as $e_1$, $e_2$ and $e_3$ in Fig.~\ref{fig:inf_graph}(b)) to obtain a new topology that has a bridge and whose tree partition now consists of two regions of comparable size. The new influence graph is shown in Fig.~\ref{fig:inf_graph}(b). One can see that, compared to the original influence graph in Fig.~\ref{fig:inf_graph}(a), the new influence graph is much less dense and, in particular, there are no edges connecting transmission lines that belong to different tree partition regions. We also note that the network in Fig.~\ref{fig:inf_graph}(b) contains two cut vertices (indicated by $c_1$ and $c_2$ in the figure, with $c_2$ being created when we switch off the lines). It can be checked that line failures are ``blocked'' by these cut vertices, which verifies our results in Section \ref{section:non-bridge}.

It is also of interest to see how the network congestion is impacted by switching off these lines. To do so, we collect statistics on the difference between the branch flows in Fig.~\ref{fig:inf_graph}(b) and those in \ref{fig:inf_graph}(a). In Fig.~\ref{fig:lineflowscomparison}(a), we plot the histogram of such branch flow differences normalized by the original branch flow in Fig.~\ref{fig:inf_graph}(a). It shows that roughly half (the exact percentage is $47.41\%$) of the transmission lines have higher congestion yet the majority of these branch flow increases are negligible. To more clearly see how much the congestion becomes worse on these lines, we plot the cumulative distribution function of the normalized
positive branch flow changes, which is shown in Fig.~\ref{fig:lineflowscomparison}(b). One can see from the figure that $90\%$ of the the branch flows increase by no more than $10\%$. 

\begin{figure}
\centering
\iftoggle{isarxiv}{
\subfloat[]{\includegraphics[width=.24\textwidth]{histogram.png}
}
\subfloat[]{\includegraphics[width=.24\textwidth]{cdf.png}
}
}{
\subfloat[]{\includegraphics[width=.24\textwidth]{figs/histogram.png}
}
\subfloat[]{\includegraphics[width=.24\textwidth]{figs/cdf.png}
}
}
\caption{(a) Histogram of the normalized branch flow changes. (b) Cumulative distribution function of the positive normalized branch flow changes. Note that the curve intercepts the $y$-axis since $52.59\%$ of the branch flows decrease.}
	\label{fig:lineflowscomparison}
\end{figure}

==> converse_failure_proof.tex <==
In order to prove the desired result, we first establish a lemma that pertains the branch flow directions on all edges under a specific type of injections. More concretely, given an edge $e=(i,j)\in\calE$, we can define its ``characteristic'' injection $p^e$ by
$$
p^e_k=\begin{cases}
1, \quad & k=i,\\
-1, \quad & k=j,\\
0, & \text{otherwise}.\\
\end{cases}
$$
The following result shows that the sign of the branch flow on $\hat{e}$ under $p^e$ is determined by $D_{\hat{e}e}$, the generation shift sensitivity factor between $e$ and $\hat{e}$ (see Section \ref{section:gdf}).
\begin{lemma}\label{lemma:flow_sign}
Under the injections $p^e$, for any $\hat{e}=(w,z)\in\calE$ we have
$$
f_{\hat{e}}=D_{\hat{e}e}.
$$
\end{lemma}
\begin{proof}
From the DC power flow equations we have $f_{\hat{e}}=B_{\hat{e}}(\theta_w - \theta_z)$, where $\theta=Ap$ is the phase angles vector (with $\theta_n=0$ for the reference bus $n$). By expanding the matrix products and noting that $A$ is symmetric, we see that
$$
f_{\hat{e}} = B_{\hat{e}}(A_{iw}+A_{jz}-A_{iz}-A_{jw}) = D_{\hat{e}e}. \qedhere
$$
\end{proof}
In particular, for the edge $e$, we know $f_e=D_{ee}=B_eR_e>0$, where $R_e$ is the effective reactance of $e$, which agrees with our intuition.

Now let us consider the case $K_{\hat{e}e}>0$. When this holds, under the injection $p^e$, we have $f_e>0$ and $f_{\hat{e}} >0$ from Lemma \ref{lemma:flow_sign}. Choose a line capacity vector $\ol{f}$ so that the capacity at $\hat{e}$ is exactly at $f_{\hat{e}}$ and the capacities for other edges are sufficiently large  in the sense that these lines operate safely before and after tripping $e$. One example of $\ol{f}$ is given by
$$
\ol{f}_{u}:=\begin{cases}
f_{\hat{e}}, \quad & u=\hat{e}\\
(1+\norm{K}_{\infty})\norm{f}_{\infty}, & \text{otherwise},
\end{cases}
$$
where $\norm{\cdot}_{\infty}$ denotes the sup norm. With this choice of capacities, before tripping $e$, it is easy to see that $f$ is a safe operating point under $\ol{f}$. Further, after we trip $e$ from $\calG$, for any edge $u$ other than $\hat{e}$, the new flow satisfies
\begin{IEEEeqnarray*}{rCl}
\abs{f'_u}&=&\abs{f_u+K_{ue}f_e}\\
&\le & \abs{f_u}+\abs{K_{ue}}\abs{f_e}\\
&\le & \norm{f}_{\infty} + \norm{K}_{\infty}\norm{f}_{\infty}\\
&=&\ol{f}_u,
\end{IEEEeqnarray*}
and for $\hat{e}$ we have
$$
\abs{f'_{\hat{e}}}=\abs{f_{\hat{e}}+K_{\hat{e}e}f_e}=f_{\hat{e}}+K_{\hat{e}e}f_e>\ol{f}_{\hat{e}},
$$
where the second equality is because $f_{e}, f_{\hat{e}}, K_{\hat{e}e} >0$. In other words, after power redistributes over the new graph $\calG':=(\calN,\calE\bs\set{e})$, the branch flow on $\hat{e}$ is over its capacity yet all other lines stay within the safe range. As a result, $\hat{e}$ would be tripped in the next stage.

The case $K_{\hat{e}e}<0$ is analogous. In particular, for this case we have $f_e>0$, $f_{\hat{e}}<0$ and hence 
$$f_{\hat{e}}+K_{\hat{e}e}f_e<f_{\hat{e}}.$$
The remaining argument follows a similar construction to the case $K_{\hat{e}e}>0$. The desired result then follows.
\qed

==> effective_reactance.tex <==
The Laplacian matrix $L$ appears in circuit analysis as the admittance matrix (with a different weight), which explicitly relates the voltage and current vector in an electrical network \cite{dorfler2013kron}. In particular, given a networked resistors, it is shown in \cite{dorfler2013kron} that the effective resistance between two nodes $i$ and $j$ can be computed as
\begin{equation}\label{eqn:prem_effective_reactance}
R_{ij}:=L^\dagger_{ii}+L^\dagger_{jj}-L^\dagger_{ij}-L^\dagger_{ji}
\end{equation}
where $L^\dagger$ is the Penrose-Moore pseudoinverse of $L$. Following a similar calculation, we can show that \eqref{eqn:prem_effective_reactance} also gives the effective reactance between the buses $i$ and $j$ in a power system. That is, assuming we connect the buses $i$ and $j$ to an external probing circuit, when there is no other injection in the network, the power flow $f_{ij}$ (from the external circuit) into bus $i$ and out from bus $j$ (into the external circuit) is given as
$$
f_{ij}=\frac{\theta_i-\theta_j}{R_{ij}}
$$
and therefore the network can be equivalently reduced to a single line with reactance $R_{ij}$. If $(i,j)\in\calE$, that is $i$ and $j$ are directly connected, then physical intuition suggests
$$
R_{ij} < X_{ij}
$$
where $X_{ij}:= 1/B_{ij}$ is the reactance of line $(i,j)$, as connections from the network should only decrease the overall reactance. We show in Section \ref{section:prem_inversion} that $X_{ij}-R_{ij}$ also carries graphical meaning, proving its nonnegativity rigorously.

==> implications.tex <==
\subsection{Generation Shift Sensitivity Factor}
As another application of Proposition \ref{prop:prem_basis}, we now derive an alternative formula for the generation shift sensitivity factor \cite{wood1996generation}, that is widely studied in power system analysis literature and is defined as follows: For a pair of buses $i,j$ and an edge $e=(w,z)$, suppose we shift injection of amount $\delta p$ from $i$ to $j$, then the branch flow on $e$ changes accordingly by the DC power flow equations \eqref{eqn:prem_dc}. Denote such branch flow change by $\delta f_e$. The generation shift sensitivity factor between the pair of buses $i,j$ and the edge $e$ is defined to be the ratio between such changes:
$$
D_{ij,e}:=\frac{\delta f_e}{\delta p}
$$
Under DC power flow \eqref{eqn:prem_dc}, $D_{ij,e}$ is fully determined by the matrix $A$, and can be computed as (see \cite{wood1996generation}):
$$
D_{ij,e} = A_{iw} + A_{jz} - A_{iz}- A_{jw}
$$
\begin{cor}\label{cor:prem_cross_product}
  For $i,j,w,z\in\calN$ that are different from the slack bus, we have
  \begin{IEEEeqnarray*}{rCl}
  A_{iw} + A_{jz} - A_{iz}- A_{jw} &=&\frac{1}{\sum_{E\in \calT_\calE}\chi(E)}
  \paren{\sum_{E\in \calT(\set{i,w},\set{j,z})}\chi(E)-\sum_{E\in \calT(\set{i,z},\set{j,w})}\chi(E)}
  \end{IEEEeqnarray*}
\end{cor}
Note that this result holds regardless of whether $(w,z)$ is an edge in $\calE$ or not. Please refer to Section \ref{section:prem_proofs} for its proof.

Corollary \ref{cor:prem_cross_product} tells us that the impact of shifting generations from $i$ to $j$ propagates to the edge $e=(w,z)$ through trees that connect these endpoints. It suggests an interesting observation that, if such trees can be prevented from being formed, we can in fact ``eliminate'' the impact of the generation shift from $i$ to $j$ on the edge $e$. This observation, when interpreted in a different setting, motivates all of our results in disruption localization in Chapter \ref{chapter:localizability}.

\subsection{Effective Reactance}
The Laplacian matrix $L$ appears in circuit analysis as the admittance matrix (with a different weight), which explicitly relates the voltage and current vector in an electrical network \cite{dorfler2013kron}. In particular, given a networked resistors, it is shown in \cite{dorfler2013kron} that the effective resistance between two nodes $i$ and $j$ can be computed as
\begin{equation}\label{eqn:prem_effective_reactance}
R_{ij}:=L^\dagger_{ii}+L^\dagger_{jj}-L^\dagger_{ij}-L^\dagger_{ji}
\end{equation}
where $L^\dagger$ is the Penrose-Moore pseudoinverse of $L$. Following a similar calculation, we can show that \eqref{eqn:prem_effective_reactance} also gives the effective reactance between the buses $i$ and $j$ in a power system. That is, assuming we connect the buses $i$ and $j$ to an external probing circuit, when there is no other injection in the network, the power flow $f_{ij}$ (from the external circuit) into bus $i$ and out from bus $j$ (into the external circuit) is given as
$$
f_{ij}=\frac{\theta_i-\theta_j}{R_{ij}}
$$
and therefore the network can be equivalently reduced to a single line with reactance $R_{ij}$. If $(i,j)\in\calE$, that is $i$ and $j$ are directly connected, then physical intuition suggests
$$
R_{ij} < X_{ij}
$$
where $X_{ij}:= 1/B_{ij}$ is the reactance of line $(i,j)$, as connections from the network should only decrease the overall reactance. We show in Section \ref{section:prem_inversion} that $X_{ij}-R_{ij}$ also carries graphical meaning, proving its nonnegativity rigorously.

As a concluding example, we derive a result using Corollary \ref{cor:prem_cross_product} that relates the effective reactance $R_{ij}$ introduced in Section \ref{section:prem_laplace} to the ``tree distributions'' of $\calG$. To do so, we need the following relation between $L^\dagger$ and $A$, which is also proved in Section \ref{section:prem_proofs}:
\begin{lemma}\label{lemma:prem_l_a_equiv}
For $(i,j)\in\calE$ such that $i\neq n$, $j\neq n$, we have
$$
L^\dagger_{ii}+L^\dagger_{jj}-L^\dagger_{ij}-L^\dagger_{ji}=A_{ii}+A_{jj}-A_{ij}-A_{ji}
$$
\end{lemma}
In other words, we can replace the $L^{\dagger}$'s in \eqref{eqn:prem_effective_reactance} by the matrix $A$. 
\begin{cor}\label{cor:prem_effective_reactance}
For $(i,j)\in\calE$ such that $i\neq n$, $j\neq n$, we have
  $$
 X_{ij}-R_{ij}=X_{ij}\cdot\frac{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)}
  $$
  In particular, we always have $X_{ij}\ge R_{ij}$ and the inequality is strict if the graph after removing $(i,j)$ is connected.
\end{cor}
\begin{proof}

By taking $w=i$, $z=j$ in Corollary \ref{cor:prem_cross_product} and applying Lemma \ref{lemma:prem_l_a_equiv}, we see that
$$
R_{ij}=A_{ii}+A_{jj}-2A_{ij}=\frac{\sum_{E\in\calT(\set{i},\set{j})}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)}
$$
For each forest in $\calT(\set{i},\set{j})$, we can add the edge $(i,j)$ to form a spanning tree passing through $(i,j)$. Conversely, each spanning tree passing through $(i,j)$ after removing the edge $(i,j)$ produces a forest in $\calT(\set{i},\set{j})$. This by the definition of $\chi(E)$ implies
$$
\sum_{E\in\calT(\set{i},\set{j})}\chi(E)=X_{ij}\sum_{E\in\calT'}\chi(E)
$$
where $\calT'$ denotes the set of all spanning trees passing through $(i,j)$. This implies
\begin{IEEEeqnarray*}{rCl}
X_{ij}-R_{ij}&=&X_{ij}\cdot\frac{\sum_{E\in \calT_\calE}\chi(E)-\sum_{E\in\calT'}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)}\\
&=&X_{ij}\cdot\frac{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)}
\end{IEEEeqnarray*}
\end{proof}

This result tells us that for an edge $(i,j)$, the reduction ratio of its reactance coming from the network is precisely the (weighted) portion of spanning trees not passing through $(i,j)$ among all spanning trees. Thus more connections from the network leads to more reduction in the effective reactance on $(i,j)$, which agrees with our physical intuition.

We remark that this reactance reduction ratio is closely related to the spanning tree centrality measure \cite{teixeira2013spanning}. Indeed, from the very definition of spanning tree centrality, we have
$$
\frac{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)} + c_{(i,j)} = 1
$$
where $c_{(i,j)}$ denotes the spanning tree centrality of $(i,j)$. As a result,
$$
R_{ij} = X_{ij}c_{(i,j)}
$$
or in other words, in a power redistribution setting, the spanning tree centrality of a line precisely captures the ratio between its effective reactance and its physical line reactance.

\subsection{Line Outage Distribution Factor}\label{section:lodf}
The most relevant quantity in understanding the power redistribution in a cascading failure process is the line outage redistribution factor \cite{wood1996generation}, which we denote as $K_{e\hat{e}}$. When the line $e$ is tripped, $K_{e\hat{e}}$ is the ratio between the branch flow change over line $\hat{e}$ and the original branch flow on $e$ before it is tripped. Writing $e=(i,j), \hat{e}=(w,z)$ with $i,j,w,z\in\calN$, the constant $K_{e\hat{e}}$ is explicitly given as \cite{wood1996generation}
$$
K_{e\hat{e}}=\frac{x_e}{x_{\hat{e}}}\frac{A_{iw}+A_{jz}-A_{jw}-A_{iz}}{x_e-(A_{ii}+A_{jj}-A_{ij}-A_{ji})}
$$

We are now ready to derive an alternative formula for $K_{e\hat{e}}$.
\begin{thm}\label{thm:redist_factor}
Let $e=(i,j), \hat{e}=(w,z)$ be edges with $i,j,w,z\in\calN$. We have
\begin{equation}\label{eqn:redist_factor}
K_{e\hat{e}}=\frac{1}{x_{\hat{e}}}\frac{\sum_{E\in \calT(\set{i,w},\set{j,z})}\chi(E)-\sum_{E\in \calT(\set{i,z},\set{j,w})}\chi(E)}{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}
\end{equation}
\end{thm}
\begin{proof}
This follows from dividing the equation in Corollary \ref{cor:cross_product} by the equation in Corollary \ref{cor:effective_reactance}.
\end{proof}
Despite the complexity of \eqref{eqn:redist_factor}, all terms in this formula carry clear meanings, as we now explain.

We first focus on the numerator of \eqref{eqn:redist_factor}, in which the sum is over the spanning forests $\calT(\set{i,w},\set{j,z})$ and $\calT(\set{i,z},\set{j,w})$. Each element in $\calT(\set{i,w}, \set{j,z})$, as illustrated in Fig.~\ref{fig:spectral_correlation}, specifies a way to connect $i$ to $w$ and $j$ to $z$ through trees and captures a possible path for edge $(i,j)$ to ``spread'' impact to $(w,z)$. Similarly, elements in $\calT(\set{i,z},\set{j,w})$ captures possible paths for edge $(i,j)$ to ``spread'' impact to $(z,w)$, which counting orientation, contributes negatively to $K_{e\hat{e}}$. Therefore the numerator in \eqref{eqn:redist_factor} says that in power redistribution, the impact of line $e$ is passed to $\hat{e}$ through all possible spanning tree paths connecting $e$ and $\hat{e}$, counting orientation. The relative strength of the positive and negative impacts determines the sign of $K_{e\hat{e}}$.

Comparing \eqref{eqn:redist_factor} and Corollary \ref{cor:cross_product}, we see that the signs of $K_{e\hat{e}}$ and $\ip{e}{\hat{e}}_A$ are the same\footnote{We overload the notation $\ip{e}{\hat{e}}_A$ to represent $\ip{u_{ij}}{u_{wz}}_A$, where $e=(i,j)$ and $\hat{e}=(w,z)$.}. Thus the spectral correlation between two edges precisely captures the relative strength of the positive and negative impacts from $e$ to $\hat{e}$. When the two impacts are of equal strength, $e$ and $\hat{e}$ are spectrally orthogonal. Such intuition allows us to decide the sign of $K_{e\hat{e}}$ in certain cases without any computation. For example, in the ring network shown in Fig.~\ref{fig:ring}, by inspecting the graph, we conclude that
$$
K_{e_1e_s}<0, \quad s=2,3,4,5,6
$$
as $e_1$ can only spread negative impacts to other lines.
\begin{figure}
\centering
\iftoggle{isarxiv}{
\includegraphics[scale=.3]{ring}
}{
\includegraphics[scale=.3]{figs/ring}
}
\caption{A ring network with clockwise orientation.}\label{fig:ring}
\end{figure}

Now we focus on the denominator of \eqref{eqn:redist_factor}, in which the sum is over all spanning trees that do not pass through $(i,j)$. Each tree of this type specifies an alternative path that power can flow through if $(i,j)$ is tripped. When there are more trees of this type, the network has better ability in absorbing the impact of $(i,j)$ being tripped. Therefore the denominator of \eqref{eqn:redist_factor} precisely says that the impact of $(i,j)$ being tripped to other lines is inversely proportional to the sum of all alternative tree paths in the network. The $1/x_{\hat{e}}$ constant in \eqref{eqn:redist_factor} captures the intuition that lines with larger reactance tend to be more robust against failures of other lines.

The formula \eqref{eqn:redist_factor} does not exhibit computational advantage comparing to existing numerical methods for computing $K_{e\hat{e}}$. The significance of this result lies in its implication in structural properties of power flow redistribution and the fact that it allows us to make general inferences by simply looking at the network topology. As an example, we deduce the following result from \eqref{eqn:redist_factor}, which is also shown in \cite{lai2013allerton}, but with longer proof.
\begin{cor}
For adjacent lines $e=(i,j)$ and $\hat{e}=(i,k)$ with $i,j,k\in\calN$, we have
$$
K_{e\hat{e}}\ge 0
$$
\end{cor}
\begin{proof}
For such $e$ and $\hat{e}$, the negative term in the numerator of \eqref{eqn:redist_factor} is over the empty set and thus equals to $0$.
\end{proof}

==> laplace_solvability_proof.tex <==
As we discussed in Section \ref{section:preliminaries}, the Laplacian matrix $L:=CBC^T$ of a connected graph $\calG=(\calN,\calE)$ has rank $n - 1$, and $Lx=b$ is solvable if and only if $\bff{1}^Tb=0$, where $\bff{1}$ is the vector with a proper dimension that consists of ones. Moreover, the kernel of $L$ is given by $\spann(\bff{1})$.

If $\calN_1$ is the only region in $\calP$, then $b=0$ since $b_j=0$ for all $j\in\calN_1$. We thus know the solution space to $Lx=b$ is exactly the kernel of $L$, and the desired result holds.

If $\calN_1$ is not the only region in $\calP$, then we can find a bus that does not belong to $\calN_1$, say bus $z$. 
Without loss of generality, assume the bus $z\in\calN_k$ and corresponds to the last row and column in $L$.
Consider a solution $x$ to $Lx=b$. Since the kernel of $L$ is $\spann(\bff{1})$,  we can without loss of generality assume that the last component of $x$ is $0$. Let $\ol{L}$ be the submatrix of $L$ obtained by removing its last row and last column, and similarly let $\ol{x}$ and $\ol{b}$ be the vectors obtained by removing the last component of $x$ and $b$, respectively. Then $\ol{L}$ is invertible, and we have
$$
\ol{L}\ol{x}=\ol{b}.
$$

Denote the matrix obtained by deleting the $l$-th row and $i$-th column of $\ol{L}$ by $\ol{L}^{li}$, then by Proposition \ref{prop:prem_basis} we have
\begin{equation}\label{eqn:graph_interpretation}
\det\paren{\ol{L}^{li}}=(-1)^{l+i}\sum_{E\in\calT(\set{l,i}, \set{z})}\chi(E),
\end{equation}
where $\chi(E)=\prod_{e\in E} B_e$ and $\calT(\set{l,i}, \set{z})$ is the set of spanning forests of $\calG$ that consists of exactly two trees containing $\set{l,i}$ and $\set{z}$, respectively.

To state some useful results derived from  \eqref{eqn:graph_interpretation}, we introduce the following definition of directly connected regions:
\begin{defn}
For a tree partition $\calP=\set{\calN_1,\calN_2,\cdots, \calN_k}$ of $\calG$, we say $\calN_v$ and $\calN_w$ are \emph{\textbf{directly connected without $\calN_l$}} if the path from $\calN_v$ to $\calN_w$ in $\calG_\calP$ does not contain $\calN_l$. 
\end{defn}
The path from $\calN_v$ to $\calN_w$ in the above definition is unique since $\calG_\calP$ forms a tree. As an example, in Fig.~\ref{fig:tree_partition}, $\calN_1$ and $\calN_2$ are directly connected without $\calN_3$, while $\calN_2$ and $\calN_3$ are not directly connected without $\calN_1$.

In the following proofs we need to refer to paths in both the original graph $\calG$ and the reduced graph $\calG_\calP$. To clear potential confusions, we introduce the following terminology. Given two sets of nodes $\calN_v$ and $\calN_w$ (that can be different from the tree-partition regions in $\calP$) of $\calG$, a path in $\calG$ from $\calN_v$ to $\calN_w$ refers to a path consisting of nodes (and lines) from the original graph $\calG$ whose starting node belongs to $\calN_v$ and ending node belongs to $\calN_w$. Given two tree-partition regions $\calN_v$ and $\calN_w$, a path in $\calG_\calP$ from $\calN_v$ to $\calN_w$ refers to a path consisting of nodes (and lines) from the reduced graph $\calG_\calP$ whose starting node is $\calN_v$ and ending node is $\calN_w$. Since there is a natural correspondence between bridges in $\calG$ and lines in $\calG_\calP$, if a line $e$ in $\calG_\calP$ is contained in a path $P$ in $\calG_\calP$, we also say the corresponding bridge $\tilde{e}$ from $\calG$ is contained in $P$.

\begin{lemma}\label{lemma:not_directly_connected}
Assume $\calN_2$ and $\calN_k$ are not directly connected without $\calN_1$. If $l_1,l_2\in\calN_2$, $z\in\calN_k$ and $i\in \ol{\calN}_1$, then
$$
\calT(\set{l_1,i}, \set{z}) = \calT(\set{l_2,i},\set{z}).
$$
\end{lemma}
\begin{proof}
The path from $\calN_1$ to $\calN_2$ in $\calG_\calP$ contains a bridge in $\calG$ that incidents to $\calN_1$. Denote this bridge as $\tilde{e}$ and let $w$ be the endpoint of $\tilde{e}$ that is not in $\calN_1$. Then it is easy to check that $w$ is a cut node that any path from $\ol{\calN}_1$ to $\calN_2$ in $\calG$ must contain.

Since $\calN_2$ and $\calN_k$ are not directly connected without $\calN_1$, the path from $\calN_2$ to $\calN_k$ in $\calG_\calP$ passes through $\calN_1$. In other words, any path in $\calG$ from $\calN_2$ to $\calN_k$ must pass through a certain node in $\calN_1$, and thus contains a sub-path in $\calG$ from $\calN_1$ to $\calN_2$. This implies that $w$ is contained in any path in $\calG$ from $\calN_2$ to $\calN_k$.

Note that any tree containing $i\in\ol{\calN}_1$ and $l_1\in\calN_2$ induces a path in $\calG$ from $\ol{\calN}_1$ to $\calN_2$ and thus contains $w$. Further, any tree containing $l_2\in\calN_2$ and $z\in\calN_k$ induces a path from $\calN_2$ to $\calN_k$ in $\calG$, and thus also contains $w$. As a result, these two types of trees always share a common node $w$ and cannot be disjoint:
$$
\calT(\set{l_1,i}, \set{l_2,z})= \emptyset.
$$
Similarly ,
$$\calT(\set{l_2,i}, \set{l_1,z})= \emptyset.$$
Therefore,
\begin{IEEEeqnarray*}{rCl}
&&\calT(\set{l_1,i}, \set{z})\\
&=&\calT(\set{l_1, l_2, i}, \set{z})\sqcup\calT(\set{l_1,i}, \set{l_2, z})\\
&=&\calT(\set{l_1, l_2, i}, \set{z})\sqcup\calT(\set{l_2,i}, \set{l_1, z})\\
&=&\calT(\set{l_2,i}, \set{z}),
\end{IEEEeqnarray*}
where $\sqcup$ means disjoint union. The desired result then follows.
\end{proof}
\begin{lemma}\label{lemma:directly_connected}
Assume $\calN_2$ and $\calN_k$ are directly connected without $\calN_1$. If $l\in\calN_2$ and $i_1, i_2 \in\ol{\calN_1}$, then
$$
\calT(\set{l,i_1}, \set{z}) = \calT(\set{l,i_2},\set{z}).
$$
\end{lemma}
\begin{proof}
The path from $\calN_1$ to $\calN_k$ in $\calG_\calP$ (denoted as $P_1$) contains a bridge in $\calG$ that incidents to $\calN_1$. Denote this bridge as $\tilde{e}$ and let $w$ be the endpoint of $\tilde{e}$ that does not belong to $\calN_1$. Then it is easy to check that $w$ is a cut node that any path in $\calG$ from $\ol{\calN}_1$ to $\calN_k$ must pass through.

We claim that if $\calN_2$ and $\calN_k$ are directly connected without $\calN_1$, then any path from $\ol{\calN}_1$ to $\calN_2$ in $\calG$ must also contain $w$. Indeed, suppose not, then the path from $\calN_1$ to $\calN_2$ in $\calG_\calP$ (denoted as $P_2$) contains a bridge in $\calG$ that incidents to $\calN_1$, and this bridge is different from $\tilde{e}$. If $P_1$ and $P_2$ do not have any common super nodes, then concatenating the two paths induces a path in $\calG_\calP$ from $\calN_2$ to $\calN_k$ that passes through $\calN_1$. In other words, the path from $\calN_2$ to $\calN_k$ in $\calG_\calP$ passes through $\calN_1$, contradicting the assumption that $\calN_2$ and $\calN_k$ are directly connected without $\calN_1$. Therefore, $P_1$ and $P_2$ share a common node, say $\calN_3$. However, $P_1$ and $P_2$ induce two different sub-paths in $\calG_\calP$ from $\calN_1$ to $\calN_3$, contradicting the assumption that $\calG_\calP$ forms a tree. We thus have proved the claim.
 
Finally, note that any tree containing $i_1\in\ol{\calN}_1$ and $l\in\calN_2$ induces a path in $\calG$ from $\ol{\calN}_1$ to $\calN_2$ and thus contains $w$. Further, any tree containing $i_2\in\ol{\calN}_1$ and $z\in\calN_k$ induces a path in $\calG$ from $\ol{\calN}_1$ to $\calN_k$ and thus contains $w$. Therefore these two types of trees always share a common node $w$ and cannot be disjoint:
$$
\calT(\set{l,i_1},\set{i_2, z})=\emptyset.
$$
Similarly 
$$\calT(\set{l,i_2},\set{i_1, z})=\emptyset.$$
As a result,
\begin{IEEEeqnarray*}{rCl}
&&\calT(\set{l,i_1}, \set{z})\\
&=&\calT(\set{l,i_1, i_2}, \set{z})\sqcup\calT(\set{l,i_1}, \set{i_2, z})\\
&=&\calT(\set{l,i_1, i_2}, \set{z})\\
&=&\calT(\set{l,i_1, i_2}, \set{z})\sqcup\calT(\set{l,i_2}, \set{i_1, z})\\
&=&\calT(\set{l,i_2}, \set{z}).
\end{IEEEeqnarray*}
\end{proof}

Now since $b_k=\ol{b}_k=0$ for all $k\in\calN_1$, by Cramer's rule, we have
\begin{equation}\label{eqn:component_inversion}
x_i=\ol{x}_i=\frac{\sum_{l\notin \calN_1}(-1)^{l+i}b_l\det\paren{\ol{L}^{li}}}{\det\paren{\ol{L}}}
\end{equation}
for all $i$.

Let $\calP_1$ be set of the regions in $\calP$ that are not directly connected to $\calN_k$ without $\calN_1$ and let $\calP_2$ be the remaining regions. For a region $\calN_l\in\calP_1$, let
$$
\chi(\calN_l):=\sum_{E\in\calT(\set{\tilde{l},i},\set{z})}\chi(E),
$$
where $\tilde{l}$ is an arbitrary bus in $\calN_l$. $\chi(\calN_l)$ is well-defined by Lemma \ref{lemma:not_directly_connected}. This fact, together with the assumption $\sum_{j\in\calN_l}b_j=0$, then implies
\begin{IEEEeqnarray*}{rCl}
&&\sum_{\tilde{l}\in \calN_l}(-1)^{\tilde{l}+I}b_{\tilde{l}}\det\paren{\ol{L}^{\tilde{l}i}}\\
&=&\sum_{\tilde{l}\in \calN_l}b_{\tilde{l}}\paren{\sum_{E\in\calT(\set{\tilde{l},i},\set{z})}\chi(E)}=\sum_{\tilde{l}\in \calN_l}b_{\tilde{l}}\chi(\calN_l)\\
&=&\chi(\calN_l)\sum_{\tilde{l}\in\calN_l}b_{\tilde{l}} = 0.
\end{IEEEeqnarray*}

As a result
\begin{IEEEeqnarray*}{rCl}
&&\sum_{\tilde{l}\notin \calN_1}(-1)^{\tilde{l}+i}b_{\tilde{l}}\det\paren{\ol{L}^{\tilde{l}i}}\\
&=&\sum_{\calN_l\in\calP_1}\sum_{\tilde{l}\in\calN_l}(-1)^{\tilde{l}+i}b_{\tilde{l}}\det\paren{\ol{L}^{\tilde{l}i}}\\
&&+\sum_{\calN_l\in\calP_2}\sum_{\tilde{l}\in\calN_l} (-1)^{\tilde{l}+i}b_{\tilde{l}}\det\paren{\ol{L}^{\tilde{l}i}}\\
&=&\sum_{\calN_l\in\calP_2}\sum_{\tilde{l}\in\calN_l} (-1)^{\tilde{l}+i}b_{\tilde{l}}\det\paren{\ol{L}^{\tilde{l}i}}\\
&=&\sum_{\calN_l\in\calP_2}\sum_{\tilde{l}\in\calN_l}b_{\tilde{l}}\paren{\sum_{E\in\calT(\set{\tilde{l},i},\set{z})}\chi(E)},
\end{IEEEeqnarray*}
which by Lemma \ref{lemma:directly_connected} takes the same value for all $i\in\ol{\calN}_1$. In other words, equation \eqref{eqn:component_inversion} takes the same value for all $i\in\ol{\calN}_1$, completing the proof. \qed


==> max_flow_proof.tex <==
Thanks to the conservation constraints \eqref{eqn:flow_conservation} in DC power flow equations, for any $\calG'=(\calN,\calE')\in\mathfrak{C}$ the injection $p'$ and the branch flow $f'$ satisfies
$$
\sum_{e\in N(j)}f'_e = \begin{cases}
d,\quad &j=G,\\
-d, &j=L,\\
0, &\text{otherwise},
\end{cases}
$$
where $N(j)$ is the set of edges incident to $j$. In particular, $p'$ and $f'$ can be considered as a single ``flow'' (see \cite{west1996introduction} for the rigorous definition of such ``flow'') from $G$ to $L$ with volume $d$. Thus by the Max-Flow-Min-Cut Theorem we know for any edge cut $E\subset\calE'$,
$$
\sum_{e\in E} \abs{f_e} \ge d,
$$
and therefore, $\Psi(\calG')\ge d$. For the graph shown in Fig.~\ref{fig:double_ring}(b), the sum of absolute branch flow is exactly $d$. The desired result then follows.
\qed

==> non_bridge.tex <==
In this section, we characterize the power flow redistribution under the DC model when a non-bridge line is tripped and show that such failures are localized by the tree partition regions. More specifically, we study how the tripping of a line $e\in\calE$ impacts the branch flow on a different edge $\hat{e}\in\calE$. Recall, we mentioned in Section \ref{section:model} that when $e$ is not a bridge, the power flow change on $\hat{e}$ due to tripping $e$ is given by
\begin{equation*}
\Delta P_{\hat{e}} = K_{e\hat{e}} \times P_e.
\end{equation*}
The impact of the line failure of $e$ can thus be characterized by the distribution factor $K_{e\hat{e}}$.

\subsection{Impact across Regions}
To start with, we consider the case where $\hat{e}$ does belong to the same region as $e$, that is, $\hat{e}$ either belongs to a different region or $\hat{e}$ is a bridge. This case was studied in~\cite{guo2017monotonicity} where the following result was shown.

\begin{prop}\label{prop:disjoint_island}
Consider a power network $\calG$ with tree partition $\set{\calN_1,\calN_2,\cdots, \calN_k}$. Let $e, \hat{e}\in\calE$ be two different edges such that $e$ is not a bridge. Then,
$$
K_{e\hat{e}} = 0
$$
for any $\hat{e}$ that is not in the same the region containing $e$.
\end{prop}

This result implies that, when a non-bridge line $e$ fails, any line $\hat{e}$ not in the same tree partition region as $e$ will not be affected, regardless of whether $\hat{e}$ is a bridge. In other words, non-bridge failures cannot propagate through the boundaries formed by the tree partition regions of $\calG$.

\subsection{Impact within Regions}
It is reasonable, based on physical intuition, to expect that the converse to the above result is also true. That is, if $e, \hat{e}$ belong to a common region (and thus $e$ is not a bridge), we would expect $K_{e\hat{e}}\neq 0$. This, however, is not always the case for two reasons: (a) some vertices within a tree partition region may ``block'' spanning forests from $e$ to $\hat{e}$; (b) the graph $\calG$ may be too symmetric. We elaborate on these two scenarios separately in the following two subsections.

\subsubsection{Block Decomposition}
To illustrate the issue described above, we use the following example to demonstrate that certain vertices within a tree partition region may ``block'' spanning forests from $e$ to $\hat{e}$.

\begin{figure}
\centering
\iftoggle{isarxiv}{
\subfloat[]{\includegraphics[height=2cm]{butterfly.png}
}
\hfill
\subfloat[]{\includegraphics[height=2cm]{butterfly_decomp.png}
}
}{
\subfloat[]{\includegraphics[height=2cm]{figs/butterfly.png}
}
\hfill
\subfloat[]{\includegraphics[height=2cm]{figs/butterfly_decomp.png}
}
}
\caption{(a) A butterfly network. (b) The block decomposition of the butterfly network into cells $\calC_1$ and $\calC_2$.}\label{fig:butterfly}
\end{figure}

\begin{eg}\label{eg:butterfly}
Consider a butterfly network shown in Fig.~\ref{fig:butterfly}(a) and pick $e=(i,j)$ and $\hat{e}=(w,z)$ from the butterfly wings. It is not hard to see that any tree containing $i,w$ simultaneously must contain the body vertex $c$, and so is any tree containing $j,z$. As a result, we see $\calT\paren{\set{i,w},\set{j,z}}$ is empty. Similarly we also know $\calT\paren{\set{i,z},\set{j,w}}$ is empty. By Theorem \ref{thm:redist_factor}, we then have $K_{e\hat{e}}=0$. %\qedd
\end{eg}

The issue with Example \ref{eg:butterfly} is that the butterfly graph is not 2-connected. In other words, it is possible that the removal of a single vertex (in this case the body vertex $c$) can disconnect the original graph. We refer to such a vertex as a \emph{cut vertex} following graph-theoretic convention. From Example \ref{eg:butterfly}, we see that cut vertices may ``block'' spanning forests between edges in a tree partition region. That is, two disjoint trees cannot pass through a common cut vertex.

Fortunately, we can precisely capture such an effect by decomposing each tree partition region further through the classical \emph{block decomposition}~\cite{harary1969graph}. Recall that the block decomposition of a graph is a partition of its \emph{edges} such that each partitioned component is 2-connected. See Fig.~\ref{fig:butterfly}(b) for an illustration. We refer to such components as \emph{cells} to reflect the fact that they are smaller parts within a tree partition region. Note that two different cells within a tree partition region may share a common vertex as the block decomposition is over graph edges. The block decomposition of a graph always exists and can be found in linear time~\cite{tarjan1985efficient}.

\begin{lemma}
Consider a power network $\calG$ and let $e,\hat{e}$ be two distinct edges within the same tree partition region but across different cells. Then $K_{e\hat{e}}=0$.
\end{lemma}
\begin{proof}
Let $e=(i,j)$ be within the cell $\calC_e$ and $\hat{e}=(w,z)$ be within the cell $\calC_{\hat{e}}$. It is a classical result that any path originating from a vertex within $\calC_e$ to a vertex within $\calC_{\hat{e}}$ must pass through a common cut vertex in $\calC_e$ \cite{harary1969graph}. As a result, it is impossible to find two disjoint trees in $\calG$ containing $i,w$ and $j,z$ respectively. Thus $\calT\paren{\set{i,w}, \set{j,z}}$ is empty. Similarly $\calT\paren{\set{i,z}, \set{j,w}}$ is also empty. By Theorem \ref{thm:redist_factor}, we then know $K_{e\hat{e}}=0$.
\end{proof}

\subsubsection{Symmetry}
Next, we demonstrate that graph symmetry\footnote{By symmetry, we refer to graph automorphisms. The exact meaning of symmetry, however, is not important for our purpose.} may also block the propagation of failures.  Again, we illustrate the issue with a simple example. 

\begin{eg}\label{eg:symmetry}
Consider the complete graph on $n$ vertices and pick $e=(i,j)$ and $\hat{e}=(w,z)$ such that $e$ and $\hat{e}$ do not share any common endpoints: $i\neq j\neq w\neq z$. Assume the line susceptances are all $1$. By symmetry, it is easy to see that there is a bijective correspondence between $\calT\paren{\set{i,w},\set{j,z}}$ and $\calT\paren{\set{i,z},\set{j,w}}$, and thus
$$
\sum_{E\in \calT(\set{i,w},\set{j,z})}\chi(E)-\sum_{E\in \calT(\set{i,z},\set{j,w})}\chi(E) = 0.
$$
By Theorem \ref{thm:redist_factor}, we then have $K_{e\hat{e}}=0$.
\end{eg}

A complete graph is 2-connected and thus forms a cell. Example \ref{eg:symmetry} shows that even if the two edges $e,\hat{e}$ are within the same cell, when the graph $\calG$ is rich in symmetries, it is still possible that a failure of $e$ does not impact $\hat{e}$. Nevertheless, this issue is not critical as such symmetry almost never happens in practical systems because of heterogeneity in line susceptances. In fact, even if the system is originally symmetric, an infinitesimal change on the line susceptances is enough to break the symmetry, as we now show.

More formally, we adopt a form of perturbation analysis on the line susceptances. That is, instead of requiring the line susceptance to be fixed values $B_e$, we add a random perturbation $\omega=(\omega_e:e\in\calE)$ drawn from a probability measure $\mu$. Such perturbations can come from manufacturing error or measurement noise. The perturbed system\footnote{We assume the perturbation ensures $B_e+\omega_e > 0$ for any $e\in\calE$ so that the new susceptance is physically meaningful.} shares the same topology (and thus tree partition) as the original system, yet admits perturbed susceptances $B+\omega$. The randomness of $\omega$ implies the factor $K_{e\hat{e}}$ is now a random variable. Let $\calL_m$ be the Lebesgue measure on $\R^m$. Recall $\mu$ is \emph{absolutely continuous} with respect to $\calL_m$ if for any measurable set $S$ such that $\calL_m(S)=0$, we have $\mu(S)=0$.

\begin{prop}\label{prop:same_region}
Consider a power network $\calG$ under perturbation $\mu$ and let $e,\hat{e}$ be two distinct edges within the same cell. If $\mu$ is absolutely continuous with respect to $\calL_m$,
$$
\mu\paren{K_{e\hat{e}}\neq 0} = 1.
$$
\end{prop}
\iftoggle{isreport}{
See Appendix \ref{proof:same_region} for a proof.
}{
See our online report for a proof \cite{report}.
}

Note that, by Radon-Nikodym theorem~\cite{royden2010real}, the probability measure $\mu$ is absolutely continuous with respect to $\calL_m$ if and only if it affords a probability density function. In other words, there are no requirements on either the power or the correlation of the perturbation for Proposition \ref{prop:same_region} to apply. The only necessary condition is that the measure $\mu$ cannot contain Dirac masses. As a result, we see that for almost all practical probability models of such perturbation (e.g.,~truncated Gaussian noise with arbitrary covariance, bounded uniform distribution, truncated Laplace distribution), $K_{e\hat{e}}\neq 0$ for $e,\hat{e}$ within the same cell almost surely, no matter how small the perturbation is. 

==> proofs_new.tex <==
\section{Proofs}\label{section:prem_proofs}


==> representation.tex <==
\begin{figure}
\centering
\iftoggle{isarxiv}{
\includegraphics[width=.275\textwidth]{arxiv_figs/spanning_forest.eps}
}{
\includegraphics[width=.275\textwidth]{figs/spanning_forest.png}
}
\caption{An example element in $\calT(\calN_1,\calN_2)$, where circles correspond to elements in $\calN_1$ and squares correspond to elements in $\calN_2$. The two trees containing $\calN_1$ and $\calN_2$ are highlighted as solid lines.}\label{fig:spanning_forest}
\end{figure}

In this section, we show how the entries of the matrix $A$ are related to specific families of subtrees of the power network $\calG$. This relation reveals new perspectives on many important and well-studied quantities in contingency analysis and it is at the core of a new criterion, we call the Simple Loop Criterion, that characterizes whether the failure of a line impacts other lines. This new representation in terms of network subtrees is extensively used to develop further results in Parts II and III of this paper.

\subsection{Spectral representation}
Proposition \ref{prop:prem_laplace_tree} relates $\det(\ol{L})$ to the spanning trees of $\calG$ and hints at the fact that the subtree families of $\calG$ determine certain algebraic properties of the matrix $A$. We now present a finer-grained result that explicitly characterizes each entry of $A$ using the tree structure of $\calG$.

We first introduce some more notation. Given a subset $E \subseteq \calE$ of edges, we denote by $\calT_E$ the set of spanning trees of $\calG$ with edges from $E$ (which can possibly be empty if $E$ is too small or if $\calG$ is disconnected). In particular, $\calT_\calE$ is the set of spanning trees on $\calG$. For any pair of subsets $\calN_1, \calN_2\subset\calN$, we define $\calT(\calN_1, \calN_2)$ to be the set of spanning forests of $\calG$ consisting of exactly two trees (necessarily disjoint) that contain $\calN_1$ and $\calN_2$, respectively (see Fig.~\ref{fig:spanning_forest} for an illustration of $\calT(\calN_1, \calN_2)$). Given a subset $E \subseteq \calE$ of edges, we write
$$
\chi(E):=\prod_{e\in E}B_e.
$$
Then, the All Minors Matrix Tree Theorem \cite{chaiken1982allminor} applied to the matrix $\ol{L}$ yields the following result.
\begin{prop}\label{prop:prem_all_minor}
  The determinant of the matrix $\ol{L}^{ij}$, obtained from $\ol{L}$ by deleting the $i$-th row and $j$-th column, is equal to
  $$
  \det\paren{\ol{L}^{ij}}=(-1)^{i+j}\sum_{E\in \calT(\set{i,j},\set{n})}\chi(E).
  $$
\end{prop}
This result leads to our graphical interpretation of the elements of $A$, formally stated as follows (its proof is presented in \iftoggle{isreport}{Appendix \ref{section:spectral_rep_proof}}{our online report \cite{part1}}):
\begin{prop}[Spectral Representation]\label{prop:prem_basis}
  For any $i,j\in\calN$, 
  %such that $i,j\neq n$
  we have
  \begin{equation}\label{eqn:atom_rep}
  A_{ij}=\frac{\sum_{E\in \calT(\set{i,j},\set{n})}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)}.
  \end{equation}
\end{prop}
In the expression~\eqref{eqn:atom_rep} for $A_{ij}$, the denominator is a normalization constant common for all entries of $A$. The sum at the numerator is over the trees in $\calT(\set{i,j},\set{n})$, which means that $A_{ij}$ is proportional to the (weighted) number of trees that connect $i$ to $j$ and can be interpreted as the ``connection strength'' between the buses $i$ and $j$ in $\calG$.

The matrix $A$ fully determines the phase angles $\theta$ (and thus the branch flows $f$) from the power injections $p$ as prescribed by~\eqref{eqn:dc_model}, more specifically
$$
 \theta=A p.
$$
In view of this fact, Proposition \ref{prop:prem_basis} implies that the power redistribution under DC power flow model~\eqref{eqn:dc_model} can be described using the distribution of subtree families over the transmission network. In particular, we can deduce analytical properties of the branch flows using purely graphical structures, as we do in the following corollary.
\begin{cor}
For all $i,j\in\calN$ we have
$$
A_{ij} \ge 0,
$$
and equality holds if and only if every path from $i$ to $j$ contains the reference node $n$.
\end{cor}
\begin{proof}
The statement trivially holds when $i$ or $j$ coincides with $n$, so in the rest of the proof we focus on the case $i,j \neq n$. In this case, since $\chi(E) \ge 0$ for all $E$, we clearly have $A_{ij} \ge 0$ and equality holds if and only if the set $\calT(\set{i,j},\set{n})$ is empty.

If every path from $i$ to $j$ contains $n$, then since any tree containing $\set{i,j}$ induces a path from $i$ to $j$, we know that this tree also contains $n$. As a result, $\calT(\set{i,j}, \set{n}) = \emptyset$. Conversely, if $\calT(\set{i,j}, \set{n}) = \emptyset$, then any path from $i$ to $j$ must contain $n$, since for any path from $i$ to $j$ not passing through $n$, we can iteratively add edges that do not have $n$ as an endpoint to obtain a spanning tree over the nodes set $\calN\bs \set{n}$. This tree together with the node $n$ itself is an element of $\calT(\set{i,j}, \set{n})$. We thus have shown that $\calT(\set{i,j},\set{n})$ is empty if and only if every path from $i$ to $j$ contains $n$. %This completes the proof.
\end{proof}
In the following subsections, by making use of Proposition~\ref{prop:prem_basis}, we derive novel expressions for well-studied quantities in power system analysis, unveiling a new graphical meaning for each of them. These results allow us to derive the Simple Loop Criterion, which is the core motivation behind using the \emph{tree partitioning} of power networks for failure localization.

\subsection{Generation Shift Sensitivity Factor} \label{section:gdf}
Consider a pair of buses $i$ and $j$, which may or may not be adjacent, i.e., $(i,j)$ may or may not be an edge in $\calE$. Suppose the injection at bus $i$ is increased by $\Delta_{ij}$, the injection at bus $j$ is reduced 
by $\Delta_{ij}$, and all other injections remain unchanged so that the new injections remain balanced. Under such changes, the branch flow change $\Delta f_{\hat{e}}$ on an edge $\hat{e}$ is determined by the DC power flow equations \eqref{eqn:dc_model}.
The \textit{generation shift sensitivity factor} between the pair of buses $i,j$ and the edge $\hat{e}$ is defined as the ratio~\cite{wood1996generation} 
$$
D_{\hat{e},ij} := \frac{\Delta f_{\hat{e}}}{\Delta p}.
$$
When $e:=(i,j)\in\calE$ is an edge in the network, we also write $D_{\hat{e},ij}$ as $D_{\hat{e},e}$. 
The factor $D_{\hat{e},ij}$ is fully determined by the matrix $A$, and, if $\hat{e}=(w,z)$, it can be explicitly computed as (see \cite{wood1996generation}):
$$
D_{\hat{e},ij} = B_{\hat{e}} (A_{iw} + A_{jz} - A_{iz}- A_{jw}).
$$
Combining this formula with Proposition \ref{prop:prem_basis} yields the following result (\iftoggle{isreport}{proved in Appendix \ref{section:prem_proof_of_cross}}{see our online report \cite{part1} for a proof}):
\begin{cor}\label{cor:prem_cross_product}
  For $i,j\in\calN, \hat{e}=(w,z)\in\calE$, we have
  \begin{IEEEeqnarray*}{rCl}
D_{\hat{e},ij} &=&\frac{B_{\hat{e}}}{\sum_{E\in \calT_\calE}\chi(E)} \times
  \\
  &&\Bigg(\sum_{E\in \calT(\set{i,w},\set{j,z})}\chi(E)
  -\sum_{E\in \calT(\set{i,z},\set{j,w})}\chi(E)\Bigg).
  \end{IEEEeqnarray*}
\end{cor}

Despite its complexity, this formula carries a clear graphical meaning, as we now explain. The two sums appearing at the numerator are over the spanning forests $\calT(\set{i,w},\set{j,z})$ and $\calT(\set{i,z},\set{j,w})$ respectively. Each element in $\calT(\set{i,w}, \set{j,z})$, as illustrated in Fig.~\ref{fig:spectral_correlation}, specifies a way to connect $i$ to $w$ and $j$ to $z$ through disjoint trees and captures a possible path for $i,j$ to ``spread'' impact to $(w,z)$. Similarly, elements in $\calT(\set{i,z},\set{j,w})$ captures possible paths for $i,j$ to ``spread'' impact to $(z,w)$, which counting orientation, contributes negatively. Therefore, Corollary \ref{cor:prem_cross_product} implies that the impact of shifting generations from $j$ to $i$ propagates to the edge $\hat{e}=(w,z)$ through all possible spanning forests that connect the endpoints $i,j,w,z$ (accounting for orientation). The relative strength of the trees in these two families determines the sign of $D_{\hat{e}, ij}$.

%This intuition suggests an interesting observation that, if spanning trees that connect the endpoints $i,j,w,z$ do not exist, we can in fact completely prevent the impact of generation shifting between $i$ and $j$ from propagating to $e$. This intuition is formalized in the simple loop criteria to be presented in Section \ref{section:simple_loop}.
\begin{figure}[t]
\centering
\iftoggle{isarxiv}{
\includegraphics[width=.28\textwidth]{arxiv_figs/spectral_correlation.eps}
}{
\includegraphics[width=.28\textwidth]{figs/spectral_correlation}
}
\caption{An example element in $\calT(\set{i,w},\set{j,z})$. The spanning trees containing $\set{i,w}$ and $\set{j,z}$ are highlighted as solid lines.}\label{fig:spectral_correlation}
\end{figure}

\subsection{Effective Reactance}
The Laplacian matrix $L$ appears in circuit analysis as the admittance matrix (with a different weight), which explicitly relates the voltage and current vectors in an electrical resistive network \cite{dorfler2013kron}. In particular, given a network of resistors, it is shown in \cite{dorfler2013kron} that the \textit{effective resistance} between two nodes $i$ and $j$ can be computed as
\begin{equation}\label{eqn:prem_effective_reactance}
R_{ij}:=L^\dagger_{ii}+L^\dagger_{jj}-L^\dagger_{ij}-L^\dagger_{ji},
\end{equation}
where $L^\dagger$ is the Penrose-Moore pseudoinverse of $L$. With an analogous calculation, we can show that in our setting \eqref{eqn:prem_effective_reactance} gives the \textit{effective reactance} between the buses $i$ and $j$. This means that, assuming we connect the buses $i$ and $j$ (with phase angles $\theta_i$ and $\theta_j$ respectively) to an external probing circuit, when there are no other injections in the network, the branch flow $f_{ij}$ (from the external circuit) into bus $i$ and out of bus $j$ (into the external circuit) is given as
$$
f_{ij}=\frac{\theta_i-\theta_j}{R_{ij}}.
$$
Therefore, the network can be equivalently reduced to a single line with reactance $R_{ij}$. If $(i,j)\in\calE$, the reactance of $(i,j)$ is given as $X_{ij}:= 1/B_{ij}$. Then, the physical intuition suggests that $R_{ij} \le X_{ij}$, as additional paths from $i$ to $j$ in the network should only decrease the overall reactance. We now give a graphical interpretation for the difference $X_{ij}-R_{ij}$ and use it to prove this result rigorously.
\begin{cor}\label{cor:prem_effective_reactance}
For all $(i,j)\in\calE$ we have
  $$
 X_{ij}-R_{ij}=X_{ij}\cdot\frac{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)}.
  $$
  In particular, $X_{ij}\ge R_{ij}$ and the inequality is strict if and only if the graph $\calG$ is still connected after removing $(i,j)$.
\end{cor}
The proof of this result is presented in \iftoggle{isreport}{Appendix \ref{section:prem_effective_reactance_proof}}{our online report \cite{part1}}.
From Corollary \ref{cor:prem_effective_reactance}, we see that for an edge $(i,j)$, the reduction ratio of its reactance coming from the network is precisely the portion of weighted spanning trees not passing through $(i,j)$ among all spanning trees. 
%In other words, $R_{ij}=\frac{\sum_{E\in\calT_{ \set{(i,j)}}}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)} X_{ij}$, i.e. $R_{ij}$ is proportional to the fraction of weighted spanning trees passing through edge $(i,j)$.
Thus, more connections from the network leads to more reduction in the effective reactance on $(i,j)$, which agrees with our physical intuition.

We remark that this reactance reduction ratio is closely related to the \textit{spanning tree centrality measure} \cite{teixeira2013spanning}. Indeed,
$$
\frac{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}{\sum_{E\in \calT_\calE}\chi(E)} + c_{(i,j)} = 1,
$$
where $c_{(i,j)}$ is the spanning tree centrality of $(i,j)$. As a result
$$
R_{ij} = X_{ij}c_{(i,j)},
$$
which means that in a power network the spanning tree centrality $c_{(i,j)}$ of a transmission line $(i,j)$ precisely captures the ratio between its effective reactance $R_{ij}$ and its physical line reactance $X_{ij}$.

\subsection{Line Outage Distribution Factor}\label{section:lodf}
\begin{figure}
\centering
\iftoggle{isarxiv}{
\includegraphics[width=.18\textwidth]{arxiv_figs/ring.eps}
}{
\includegraphics[scale=.25]{figs/ring}
}
\caption{A ring network with clockwise orientation. Line $e_1$ can only spread ``negative'' impacts to other lines.}\label{fig:ring}
\end{figure}
As we discussed in Section \ref{section:preliminaries}, when a line $e$ is tripped from a power network $\calG$, the line outage distribution factor $K_{\hat{e}e}$ captures the ratio between the flow change over line $\hat{e}$ with respect to the original branch flow on $e$ before it is tripped. Writing $e=(i,j), \hat{e}=(w,z)$ with $i,j,w,z\in\calN$, the constant $K_{\hat{e}e}$ can be computed as \cite{wood1996generation}:
$$
K_{\hat{e}e}=\frac{X_e}{X_{\hat{e}}}\cdot\frac{A_{iw}+A_{jz}-A_{jw}-A_{iz}}{X_e-(A_{ii}+A_{jj}-A_{ij}-A_{ji})}.
$$
This formula only holds if the graph $\calG':=(\calN,\calE\bs\set{e})$ is connected, as otherwise its denominator is $0$ by Corollary \ref{cor:prem_effective_reactance}. An edge of the graph $\calG$ whose removal disconnects the graph is known as a \emph{bridge} in the literature. We discuss this concept and its relationship to tree partitions in more detail in Section \ref{section:basic}. 

Using our previous results, we can readily derive the following new formula for $K_{\hat{e}e}$.
\begin{thm}\label{thm:redist_factor}
Let $e=(i,j)$, $\hat{e}=(w,z)$ be edges such that $\calG':=(\calN,\calE\bs\set{e})$ is connected. Then $K_{\hat{e}e}$ is given by
\begin{equation}\label{eqn:redist_factor}
B_{\hat{e}}\times \frac{\sum_{E\in \calT(\set{i,w},\set{j,z})}\chi(E)-\sum_{E\in \calT(\set{i,z},\set{j,w})}\chi(E)}{\sum_{E\in\calT_{\calE\bs \set{(i,j)}}}\chi(E)}.
\end{equation}
\end{thm}
\begin{proof}
This result readily follows by dividing the identity in Corollary \ref{cor:prem_cross_product} by that in Corollary \ref{cor:prem_effective_reactance}.
\end{proof}
Similar to our discussions in Section \ref{section:gdf}, each term in \eqref{eqn:redist_factor} also carries clear graphical meanings: (a) The numerator of \eqref{eqn:redist_factor} states that the impact of tripping $e$ propagates to $\hat{e}$ through all possible trees that connect $e$ to $\hat{e}$, counting orientation. (b) The denominator of \eqref{eqn:redist_factor} sums over all spanning trees of $\calG$ that do not pass through $e=(i,j)$, and each tree of this type specifies an alternative path that power can flow through if $(i,j)$ is tripped. When there are more trees of this type, the network has a better ability to ``absorb'' the impact of $(i,j)$ being tripped, and the denominator of \eqref{eqn:redist_factor} precisely captures this effect by saying that the impact of $e$ being tripped on other lines is inversely proportional to the sum of all alternative tree paths in the network. (c) The $B_{\hat{e}}$ in \eqref{eqn:redist_factor} captures the intuition that a line with a larger reactance tends to be more robust against failures of other lines.

This graphical interpretation of identity~\eqref{eqn:redist_factor} allows us to make general inferences on $K_{\hat{e}e}$ using only knowledge of  the network topology. For example, in the ring network shown in Fig.~\ref{fig:ring}, by inspecting the graph, we conclude that
$$
K_{e_se_1}<0, \quad s=2,3,4,5,6,
$$
as $e_1$ can only spread ``negative'' impacts to other lines (the positive term in \eqref{eqn:redist_factor} vanishes).

From Theorem \ref{thm:redist_factor}, we recover the following result from \cite{lai2013allerton}, whose original proof is much longer.
\begin{cor}
For adjacent lines $e=(i,j)$ and $\hat{e}=(i,k)$, we have
$$
K_{\hat{e}e}\ge 0.
$$
\end{cor}
\begin{proof}
For such $e$ and $\hat{e}$, the second term in the numerator of \eqref{eqn:redist_factor} is over the empty set and thus equals to $0$.
\end{proof}

Given two edges $e$ and $\hat{e}$, $K_{\hat{e}e}$ captures how the branch flow on $\hat{e}$ changes if $e$ is tripped. In particular, if $K_{\hat{e}e}=0$, then the failure of $e$ cannot lead to successive failure of $\hat{e}$ (in one step) as the branch flow on $\hat{e}$ is not impacted. The following result shows that the converse also holds if we are allowed to choose the injection and line capacities adversarially (see  \iftoggle{isreport}{Appendix \ref{proof:converse_failure}}{our online report \cite{part1}} for its proof).
\begin{prop}\label{prop:converse_failure}
Given $e,\hat{e}\in\calE$ with $K_{\hat{e}e}\neq 0$, there exist injections $p$ and line capacities $\ol{f}$, such that before $e$ trips
$$
\abs{f_u}\le \ol{f}_u \quad \forall \, u\in\calE,
$$
while, after $e$ trips,
$$
\abs{f'_{\hat{e}}} > \ol{f}_{\hat{e}},
$$
where $f'_{\hat{e}}$ is the new flow on $\hat{e}$ over $\calG'=(\calN,\calE\bs\set{e})$.
\end{prop}
In other words, for $e$ and $\hat{e}$ such that $K_{\hat{e}e}\neq 0$, there always exists a scenario where the failure of $e$ leads to the failure of $\hat{e}$. As such, $K_{\hat{e}e}$ determines whether it is possible for the failure of $e$ to cause the failure of $\hat{e}$. The factors $K_{\hat{e}e}$'s can thus be interpreted as indicators on the system's ability to localize failures, and it is reasonable to optimize the topology $\calG$ so that $K_{\hat{e}e}=0$ for as many pairs of edges as possible.

\subsection{Simple Loop Criterion} \label{section:simple_loop}
The formula \eqref{eqn:redist_factor} shows that the spanning forests $\calT(\set{i,w},\set{j,z})$ and $\calT(\set{i,z},\set{j,w})$ fully determine if $K_{\hat{e}e}$ is $0$ or not. In other words, whether tripping $e$ has any impact on $\hat{e}$ depends on how these edges are connected by subtrees in $\calG$. We now establish an equivalent criterion that can be directly verified from the graph.

If $K_{\hat{e}e}\neq 0$, then \eqref{eqn:redist_factor} implies that at least one of the spanning forest sets $\calT(\set{i,w},\set{j,z})$ and $\calT(\set{i,z},\set{j,w})$ is nonempty. Without loss of generality, let us assume $\calT(\set{i,w},\set{j,z})\neq\emptyset$. For any element in $\calT(\set{i,w},\set{j,z})$ (see Fig.~\ref{fig:spectral_correlation}), the tree containing $\set{i,w}$ induces a path from $i$ to $w$, and the tree containing $\set{j,z}$ induces a path from $j$ to $z$. By adjoining the edges $e=(i,j)$ and $\hat{e}=(w,z)$ to these two paths, we obtain a simple loop\footnote{A loop is simple if it visits each node in the loop at most once.} containing both $e$ and $\hat{e}$. As a result, $K_{\hat{e}e}\neq 0$ implies that we can find a simple loop in $\calG$ which contains both $e$ and $\hat{e}$.

The converse, unfortunately, in general does not hold because of certain systems with high symmetry. That is, there exist pathological systems where a simple loop containing $e$ and $\hat{e}$ exists, yet $K_{\hat{e}e}=0$. Nevertheless, for such systems, by perturbing the line susceptances $B_e$ with an arbitrarily small noise, we can ``break'' the symmetry and show that $K_{\hat{e}e}\neq 0$ almost surely. The detailed technical treatments for this perturbation analysis is presented in Part II of this paper.  

The following proposition formally summarizes the discussions above:
\begin{thm}[Simple Loop Criterion]\label{prop:simple_loop}
For $e=(i,j),\hat{e}=(w,z)\in\calE$ such that $\calG':=(\calN,\calE\bs\set{e})$ is connected, we have $K_{\hat{e}e}\neq 0$ ``if'' and only if there exists a simple loop in $\calG$ that contains both $e$ and $\hat{e}$.
\end{thm}
We name this criterion ``Simple Loop'' both because it involves simple loops in $\calG$ and because it is an intuitive, hence simple, criterion depending on loops.
The ``if'' part of Theorem \ref{prop:simple_loop} should be interpreted as a probability one event under proper perturbations (see Part II of this paper for more details). This proposition shows that a simple loop containing $e$ and $\hat{e}$ must exist if tripping $e$ can possibly cause a successive failure of $\hat{e}$, since otherwise the branch flow on $\hat{e}$ is not impacted by the tripping of $e$. As a result, by clustering the network in smaller regions connected in a loop-free manner, we can prevent long-distance propagation of line failures. With this motivation in mind, in the next section we define precisely a \emph{tree partition} of a power network and study its properties.

==> same_region_proof.tex <==
Let $\calC$ be the cell that $e$ and $\hat{e}$ belong to and write $e=(i,j)$ and $\hat{e}=(w,z)$. Consider the polynomial in line susceptances $(B_e:e\in\calE)$ defined as
$$
f(B):=\sum_{E\in\calT\paren{\set{i,w}, \set{j,z}}}\chi(E)-\sum_{E\in\calT\paren{\set{i,z}, \set{j,w}}}\chi(E)
$$
We claim $f$ is not identically zero.

First, let $C$ be a simple cycle in $\calC$ that contains both $e$ and $\hat{e}$. Such a cycle always exists as $\calC$ is 2-connected by construction, and it is a classical result that any pair of edges are contained in a simple cycle for 2-connected graphs \cite{harary1969graph}. Therefore, we can find two disjoint paths $P_1$ and $P_2$ connecting the endpoints of $e$ and $\hat{e}$. Without loss of generality, assume $P_1$ connects $i$ to $w$ and $P_2$ connects $j$ to $z$. By iteratively adding edges from $\calG$ to $P_1$ and $P_2$, we can extend $P_1$ and $P_2$ to a spanning forest of $\calG$ consisting of exactly two trees. Moreover, the tree extended from $P_1$ contains $i, w$ and the tree extended from $P_2$ contains $j,z$. We thus have constructed an element of $\calT\paren{\set{i,w}, \set{j,z}}$. Denote this element by $E_0$.

Second, we show that 
$$\calT\paren{\set{i,w}, \set{j,z}}\cap \calT\paren{\set{i,z}, \set{j,w}}=\emptyset$$
Indeed, consider an element $E_1$ from $\calT\paren{\set{i,w}, \set{j,z}}$, which consists of two trees $\calT_1$ and $\calT_2$ with $\calT_1$ containing $i,w$ and $\calT_2$ containing $j,z$. If $E_1\in\calT\paren{\set{i,z}, \set{j,w}}$, then $\calT_1$ must also contain $z$. However, this implies $z\in \calT_1\cap \calT_2$, and thus $\calT_1$ and $\calT_2$ are not disjoint, contradicting the definition of $\calT\paren{\set{i,w}, \set{j,z}}$.

As a result, we see that the element $E_0$ constructed in our first step contributes a term to $\sum_{E\in\calT\paren{\set{i,w}, \set{j,z}}}\chi(E)$ but not to $\sum_{E\in\calT\paren{\set{i,z}, \set{j,w}}}\chi(E)$. Therefore $f(B)$ contains nonvanishing terms and is not identically zero.

It is well-known from algebraic geometry that the root set of a polynomial which is not identically zero has Lebesgue measure zero \cite{federer1969geometric}. That is, we have
$$
\mu\paren{f(B+\omega)=0} = \calL_m\paren{f(B+\omega)=0} = 0
$$
where the first equality is because $\mu$ is absolutely continuous with respect to $\calL_m$ (it is clear that the root set of the polynomial $f$ is measurable).

Finally, by Theorem \ref{thm:redist_factor}, we know $K_{e\hat{e}}= 0$ if and only if $f(B+\omega)=0$. This then implies
$$
\mu(K_{e\hat{e}}\neq 0) = 1 - \mu(K_{e\hat{e}}=0) = 1-\mu\paren{f(B+\omega)=0} = 1
$$
and completes our proof. \qedd

==> summary.tex <==
In the previous section, motivated by the Simple Loop Criterion, we formally introduce the notion of tree partition of a power network. 
In this section we demonstrate three localization benefits of tree partitioning: (a) It confines the impact of line outages to within their own tree-partition regions; (b) It confines the impact of certain power injection disruptions to within their own tree partition-regions; and (c) Tree partitioning can sometimes reduce, rather than increase, line congestions. We demonstrate benefits (a) and (c) using a stylized example here, and both aspects will be more extensively studied in Part II of the paper.  Benefit (b) is demonstrated by a more general result, which will also be used in Part III to design our real-time mitigation strategy for cascading failure.

\subsection{Localization of Line Failures}
Consider the double-ring network in Fig.~\ref{fig:double_ring}(a), which contains exactly one generator and one load bus, denoted by $G$ and $L$ respectively. This network admits only the trivial tree partition and the branch flows are shown in Fig.~\ref{fig:double_ring}(a). Consider a new network obtained by switching off the upper tie-line, creating a finer tree partition with two regions: the left ring and the right ring. This new network and the redistributed branch flows are shown in Fig.~\ref{fig:double_ring}(b). 

It is easy to check that in the original network Fig.~\ref{fig:double_ring}(a) there is a simple loop containing any pair of edges. The Simple Loop Criterion implies that the impact of any single-line failure in this topology is global, i.e., all the other branch flows will change almost surely.  Hence, after the single-line failure,
 every remaining line may carry a new branch flow that exceeds its capacity and subsequently trips (see~Proposition \ref{prop:converse_failure}). In contrast, for the network in Fig.~\ref{fig:double_ring}(b), there are only two loops (corresponding to the two rings). The Simple Loop Criterion guarantees that the line failures inside one ring do not impact branch flows in the other and, thus, line failures are localized within their own regions.

Such localization, however, only applies in the first stage of a cascading failure, as further failures may involve bridges in the graph, to which the Simple Loop Criterion no longer applies. In fact, as we show in Part II of this paper, tripping a bridge almost always has a global impact and, therefore, failures may still propagate from one region to another after multiple steps. Further, the newly created bridge in Fig.~\ref{fig:double_ring}(b) is a single-point vulnerability, whose failure disconnects the system into two islands. In Part III, we discuss how these drawbacks can be overcome by adopting a new control approach for fast-timescale frequency regulation.

\subsection{Localization of Injection Disruptions}
%\slow{Please check this subsection to make sure I don't miss anything.}
%\cliang{It looks good to me!}
Besides the ability to localize the impact of line failures, the tree partition of a power network also ensures that disruptions in power injections in one region do not impact another region. 
This is due to a ``decoupling'' structure of the solution space of Laplacian equations, as we now describe.
Given a tree partition $\calP=\set{\calN_1,\calN_2,\cdots, \calN_l}$ of $\calG$, for $k=1,2,\ldots, l$, let
$$
\partial\calN_k:=\set{j: j\notin\calN_k, \exists i\in\calN_k \text{ s.t. } (i,j)\in \calE \text{ or } (j,i)\in\calE}
$$
and $\ol{\calN}_k=\calN_k\cup \partial\calN_k$. The set $\partial\calN_k$ defined above consists of the \emph{boundary} buses of $\calN_k$ in $\calG$ and $\ol{\calN}_k$ can be interpreted as the \emph{closure} of $\calN_k$. As an example, in Fig.~\ref{fig:double_ring}(b), the closure of the left ring is given by the ring itself together with the bus $L$, and the closure of the right ring is given by the right ring itself together with the bus $G$.
\begin{lemma}\label{lemma:laplace_solvability}
Let $\calP=\set{\calN_1,\calN_2,\cdots, \calN_l}$ be a tree partition of $\calG$ and consider a vector $b\in\R^{n}$ such that $b_j=0$ for all $j\in\calN_1$ and $\sum_{j\in\calN_k} b_j=0$ for $k\neq 1$. Then the Laplacian equation
\begin{equation}\label{eqn:laplace_eqn}
Lx = b
\end{equation}
is solvable, and any solution $x$ of \eqref{eqn:laplace_eqn} satisfies $x_i=x_j$ for all $i,j\in\ol{\calN}_1$.
\end{lemma}
The proof of this result is presented in \iftoggle{isreport}{Appendix \ref{section:failure_proofs}}{ our online report \cite{part1}}.   
Lemma \ref{lemma:laplace_solvability} is used in Part III of this paper to design mitigation strategy that adjusts power injections 
in a way that localizes the impact of initial failures.
It implies the following region independence property in the DC power flow context: If $b$ represents perturbations in power injections, then $x$ is the resulting changes in phase angles. 
Lemma \ref{lemma:laplace_solvability} implies that the changes in phase angles are the same at every node in $\ol{\calN}_1$.
Therefore the angle difference across every line in or incident to $\calN_1$ is zero and the branch flows on these lines are 
unchanged, i.e., the branch flows in $\calN_1$ are independent of the perturbations in power injections in other regions as long as they are balanced. 

This result holds only if the regions form a tree partition. In fact, the graph in Fig.~\ref{fig:double_ring}(a) provides a counter-example when the network is not tree-partitioned: for this graph, if we set $\calN_2:=\set{G,L}$ and collect the remaining buses in $\calN_1$, then the injections satisfies the condition that $b_j=0$ for all $j\in \calN_1$ and $\sum_{j\in\calN_2}b_j=0$, yet the phase angle differences across edges in $\calN_1$ are not zero.


\subsection{Congestion Reduction}
\begin{figure}
{\centering
\iftoggle{isarxiv}{
\subfloat[]{\includegraphics[width=.22\textwidth]{arxiv_figs/double_ring.eps}}
\hspace{0.5cm}
\subfloat[]{\includegraphics[width=.22\textwidth]{arxiv_figs/double_ring_trip.eps}}
}{
\subfloat[]{\includegraphics[width=.22\textwidth]{figs/double_ring.png}}
\hspace{0.5cm}
\subfloat[]{\includegraphics[width=.22\textwidth]{figs/double_ring_trip.png}}
}}

\captionsetup{justification = justified,
              singlelinecheck = false}
\caption{(a) A double-ring network with $G$ as generator bus and $L$ as load bus, with arrows representing the original branch flow. (b) The new network after removing an edge, with arrows representing the new branch flow.}\label{fig:double_ring}
\captionsetup{size=footnotesize,
    justification=centering, %% not needed
    skip=5pt, position = bottom}
\end{figure}
It is reasonable to expect that switching off lines to refine a tree partition may increase the stress on the remaining lines and, in this way, worsens network congestion. Nonetheless, by comparing the branch flows in Fig.~\ref{fig:double_ring}(a) and (b), we notice that creating a nontrivial tree partition as in Fig.~\ref{fig:double_ring}(b) actually can potentially remove the circulating flows and hence globally reduce network congestion. 
In fact, stronger result holds in this stylized example: the tree partition in Fig.~\ref{fig:double_ring}(b) further minimizes the sum of absolute branch flows over all possible topologies on this network where $G$ and $L$ are connected. To see this, let 
$$
\mathfrak{C}:=\set{\calG'=(\calN, \calE'): G \text{ and } L \text{ are connected in }\calG'}
$$
be the collection of all graphs $\calG'=(\calN, \calE')$ with edge set $\calE'\subseteq \calN \times \calN$ (which do not need to be a sub-graph of Fig.~\ref{fig:double_ring}(a)) such that $G$ is connected to $L$ (but $G$ and $L$ are not necessarily adjacent to each other). Let $p'$ be the vector of injections described earlier, namely $p_G'=d$, $p_L'=-d$ for some $d>0$, and $p_j'=0$ for all the other buses. For each $\calG'=(\calN, \calE')\in\mathfrak{C}$, define the metric
$$
\Psi(\calG'):=\sum_{e\in\calE'}\abs{f_e'},
$$
where $f_e'$ is the branch flow on $e$ under the injection $p'$. Then we have the following result (see \iftoggle{isreport}{Appendix \ref{section:max_flow_proof}}{our online report \cite{part1}} for its proof):
\begin{prop}\label{prop:max_flow}
The graph in Fig.~\ref{fig:double_ring}(b) minimizes the sum of absolute branch flow $\Psi(\cdot)$ over $\mathfrak{C}$.
\end{prop}
Hence not only may switching off lines \emph{reduce} congestion, the tree partition in Fig.~\ref{fig:double_ring}(b) 
in fact achieves the best possible congestion reduction in terms of $\Psi(\cdot)$. We revisit this phenomenon with case studies on more complex IEEE test systems in Part II of this paper.


==> uniqueness_proof.tex <==
For $\calG=(\calN, \calE)$, let $\calE_b$ be the set of edges that all spanning trees of $\calG$ pass through. In other words, $\calE_b$ is the set of all bridges in classical graph theory. Let $\calG_b=(\calN, \calE\bs\calE_b)$ denote the graph obtained from $\calG$ by removing all edges in $\calE_b$, and let $\calP^*=\set{C_1, C_2, \cdots, C_{k}}$ be its connected components, where $k=|\calE_b|+1$. We claim $\calP^*$ is an irreducible tree partition of $\calG$.

First we show that the reduced graph $\calG_{\calP^*}$ is a tree. Assume not, then there is a loop in $\calG_{\calP^*}$. Without loss of generality, let us assume the loop is $\paren{C_{1}, C_{2}, \cdots, C_{l}}$ for some $2\le l \le k$. Then by the construction of $\calG_{\calP^*}$, there exist nodes $n_1^t, n_1^s, n_2^t, n_2^s, n_3^t, \cdots, n_l^t, n_l^s$ such that:
\begin{enumerate}
\item For each $i$, the nodes $n_i^s,n_i^t\in C_i$;
\item For each $i$, the edge $e_{i,i+_l1}:=(n_i^s, n_{i+_l1}^t) \in \calE$, where $+_l$ denotes the addition modulo $l$.
\end{enumerate}
For any $i$, since $C_i$ is connected, we can find a path $P_i$ from $n_i^t$ to $n_i^s$. It is then clear that the concatenated path
$$
\paren{P_1,e_{1,2},P_2,e_{2,3}\ldots e_{l-1,l},P_l,e_{l,1}}
$$
forms a loop in the original graph $\calG$. Consequently, not all spanning trees pass through $e_{1,2}$ and thus $e_{1,2}\notin\calE_b$, which leads to a contradiction.

Next we prove $\calP^*$ is irreducible by showing that $\calP^*$ is finer than any tree partition $\calP:=\set{\calN_1, \calN_2, \cdots, \calN_{k'}}$ of $\calG$. Consider a region in $\calP^*$, say $C_1$. Since both $\calP^*$ and $\calP$ are partitions of $\calG$, there must be some region in $\calP$, say $\calN_1$, such that $C_1\cap \calN_1\neq \emptyset$. We claim that $C_1\subset \calN_1$. Otherwise, there exists another region in $\calP$, say $\calN_2$, such that $C_1\cap \calN_2\neq \emptyset$. Pick $n_1\in C_1\cap \calN_1$ and $n_2\in C_1\cap \calN_2$. Then $n_1\neq n_2$ because $\calN_1\cap\calN_2=\emptyset$. Now since $n_1,n_2\in C_1$, and $C_1$ does not contain any bridge (in classical graph theory sense), by Menger's Theorem \cite{menger1927allgemeinen}, there exists a cycle (which is not necessarily simple) in $C_1$ containing both $n_1$ and $n_2$. By collapsing adjacent nodes in this cycle that belong to common regions, we can find regions $\calN_{l_1}^1, \calN_{l_2}^1, \cdots, \calN_{l_{p_1}}^1, \calN_{l_1}^2, \calN_{l_2}^2, \cdots, \calN_{l_{p_2}}^2$ so that the  path from $n_1$ to $n_2$ in this cycle is given by
$$
\paren{P^1_1,e_{1,l_1}^1,P^1_{l_1}, e_{l_1,l_2}^1,  \cdots, e_{l_{p_1}, 2}^1, P^1_2}
$$
and the path from $n_2$ to $n_1$ in this cycle is given by
$$
\paren{P^2_2,e_{2,l_1}^2,P^2_{l_1}, e_{l_1,l_2}^2,  \cdots, e_{l_{p_2}, 1}^2, P^2_1},
$$
where $e_{i, j}^{1}, e_{i,j}^{2}$ are edges with source nodes in $\calN_i$ and target nodes in $\calN_j$ and $P_i^1, P_i^2$ are paths contained in $\calN_i$. Therefore,
$$
\paren{\calN_1,\calN_{l_1}^1, \cdots, \calN_{l_{p_1}}^1, \calN_2, \calN_{l_1}^2, \cdots, \calN_{l_{p_2}}^2}
$$
forms a loop in $\calG_{\calP}$. This implies that $\calP$ is not a tree partition, contradicting our assumption.

We have shown that $\calP^*$ is an irreducible tree partition of $\calG$. Moreover, for any other irreducible tree partition $\ol{\calP}$, the above proof shows that
$$
\calP^*\succeq \ol{\calP}.
$$
Since $\ol{\calP}$ is irreducible and thus maximal with respect to $\succeq$, we see $\ol{\calP} = \calP^*$. In other words, any irreducible tree partition of $\calG$ must coincide with $\calP^*$. This completes our proof. \qed
